TESS Duotransit Candidates from the Southern Ecliptic Hemisphere

Discovering transiting exoplanets with long orbital periods allows us to study warm and cool planetary systems with temperatures similar to the planets in our own Solar system. The TESS mission has photometrically surveyed the entire Southern Ecliptic Hemisphere in Cycle 1 (August 2018 - July 2019), Cycle 3 (July 2020 - June 2021) and Cycle 5 (September 2022 - September 2023). We use the observations from Cycle 1 and Cycle 3 to search for exoplanet systems that show a single transit event in each year - which we call duotransits. The periods of these planet candidates are typically in excess of 20 days, with the lower limit determined by the duration of individual TESS observations. We find 85 duotransit candidates, which span a range of host star brightnesses between 8 < $T_{mag}$ < 14, transit depths between 0.1 per cent and 1.8 per cent, and transit durations between 2 and 10 hours with the upper limit determined by our normalisation function. Of these candidates, 25 are already known, and 60 are new. We present these candidates along with the status of photometric and spectroscopic follow-up.

==> 2.Methods/latex_tab.tex <==
\begin{landscape}
\begin{longtable}{ccccccccccccc}
\caption{Duotransit candidates from MonoTools fits.}\\
\toprule
TIC & $R_S$ & $\rho_S$ & $t_{0}$ & $t_{1}$ & $R_p$ & $t_{\rm D}$ & $b$ & $P_{\rm min}$ & $P_{\rm max}$ & $N_{\rm alias}$ & $P_{\rm marg}$ & $e_{\rm marg}$ \\
 & $R_\odot$ & $\rho_\odot$ & BJD-2457000 & BJD-2457000 & $R_\oplus$ & d & --- & d & d & --- & d & --- \\
\hline
193318850 &  $ 0.791 \pm 0.042 $  &  $ 1.94^{+0.5}_{-0.4} $  &  $ 1553.7698 \pm 0.0022 $  &  $ 2292.5112 \pm 0.0019 $  &  $ 7.08 \pm 0.47 $  &  $ 0.1595 \pm 0.0057 $  &  $ 0.31 \pm 0.22 $  &  $ 15.07635^{+6e-05}_{-5e-05} $  &  $ 738.7414 \pm 0.0029 $  & 50 &  $ 17.6^{+5.5}_{-2.2} $  &  $ 0.159^{+0.061}_{-0.006} $  \\
251057075 &  $ 0.839 \pm 0.053 $  &  $ 1.38^{+0.44}_{-0.32} $  &  $ 1426.3181 \pm 0.0029 $  &  $ 2154.024 \pm 0.0029 $  &  $ 3.88 \pm 0.3 $  &  $ 0.1919^{+0.0081}_{-0.0098} $  &  $ 0.27 \pm 0.22 $  &  $ 16.53877 \pm 9e-05 $  &  $ 727.7059 \pm 0.0041 $  & 45 &  $ 20.2^{+7.8}_{-3.3} $  &  $ 0.185^{+0.024}_{-0.011} $  \\
211376134 &  $ 1.114 \pm 0.052 $  &  $ 0.93 \pm 0.2 $  &  $ 1341.31106 \pm 0.00034 $  &  $ 2078.1624 \pm 0.00033 $  &  $ 27.1 \pm 2.7 $  &  $ 0.1434 \pm 0.002 $  &  $ 0.979^{+0.027}_{-0.036} $  &  $ 16.74662 \pm 1e-05 $  &  $ 736.85134 \pm 0.00047 $  & 45 &  $ 18.9^{+4.9}_{-2.1} $  &  $ 0.16^{+0.085}_{-0.029} $  \\
145006304 &  $ 1.125 \pm 0.049 $  &  $ 0.92 \pm 0.22 $  &  $ 1579.5035 \pm 0.0039 $  &  $ 2318.2439 \pm 0.004 $  &  $ 5.1 \pm 0.47 $  &  $ 0.151 \pm 0.012 $  &  $ 0.63^{+0.17}_{-0.35} $  &  $ 16.78955 \pm 0.00013 $  &  $ 738.7404 \pm 0.0057 $  & 45 &  $ 18.9^{+5.7}_{-2.2} $  &  $ 0.287^{+0.062}_{-0.022} $  \\
303317324 &  $ 0.72 \pm 0.069 $  &  $ 1.42^{+0.6}_{-0.43} $  &  $ 1365.1767 \pm 0.0028 $  &  $ 2104.3465 \pm 0.0028 $  &  $ 2.65 \pm 0.27 $  &  $ 0.2424 \pm 0.0058 $  &  $ 0.27^{+0.26}_{-0.2} $  &  $ 16.79931 \pm 9e-05 $  &  $ 739.1697 \pm 0.0039 $  & 45 &  $ 22.0^{+13.0}_{-5.0} $  &  $ 0.34 \pm 0.08 $  \\
140750416 &  $ 0.873 \pm 0.047 $  &  $ 1.49^{+0.4}_{-0.31} $  &  $ 1504.8024 \pm 0.002 $  &  $ 2245.3951 \pm 0.0013 $  &  $ 8.46 \pm 0.51 $  &  $ 0.1595^{+0.0046}_{-0.004} $  &  $ 0.36 \pm 0.22 $  &  $ 16.83165^{+6e-05}_{-5e-05} $  &  $ 740.5928 \pm 0.0024 $  & 45 &  $ 19.0^{+4.9}_{-2.2} $  &  $ 0.226^{+0.08}_{-0.036} $  \\
224279805 &  $ 1.198 \pm 0.068 $  &  $ 0.59 \pm 0.12 $  &  $ 1369.7276^{+0.0026}_{-0.0024} $  &  $ 2105.2154 \pm 0.0018 $  &  $ 10.55 \pm 0.64 $  &  $ 0.2456^{+0.0049}_{-0.0043} $  &  $ 0.24 \pm 0.18 $  &  $ 17.51161^{+8e-05}_{-7e-05} $  &  $ 735.4878 \pm 0.0032 $  & 43 &  $ 19.9^{+5.5}_{-1.9} $  &  $ 0.148^{+0.074}_{-0.016} $  \\
221915858 &  $ 2.469 \pm 0.094 $  &  $ 0.173^{+0.038}_{-0.031} $  &  $ 1643.358 \pm 0.0011 $  &  $ 2372.5512 \pm 0.0011 $  &  $ 21.3^{+3.7}_{-1.4} $  &  $ 0.1302 \pm 0.0056 $  &  $ 0.911^{+0.044}_{-0.025} $  &  $ 17.7852 \pm 4e-05 $  &  $ 729.1932 \pm 0.0015 $  & 42 &  $ 19.7^{+5.4}_{-1.9} $  &  $ 0.55^{+0.06}_{-0.027} $  \\
287204963 &  $ 1.04 \pm 0.19 $  &  $ 1.08^{+0.79}_{-0.5} $  &  $ 1402.9366 \pm 0.0025 $  &  $ 2132.3352 \pm 0.0028 $  &  $ 11.3 \pm 2.2 $  &  $ 0.1798^{+0.0097}_{-0.0078} $  &  $ 0.41^{+0.25}_{-0.28} $  &  $ 17.79021 \pm 9e-05 $  &  $ 729.3986 \pm 0.0037 $  & 42 &  $ 20.3^{+5.8}_{-2.5} $  &  $ 0.255^{+0.063}_{-0.022} $  \\
20904104 &  $ 0.881^{+0.045}_{-0.045} $  &  $ 1.35^{+0.36}_{-0.28} $  &  $ 1390.112^{+0.0039}_{-0.0048} $  &  $ 2105.3633^{+0.0037}_{-0.0033} $  &  $ 2.6 \pm 0.19 $  &  $ 0.226^{+0.02}_{-0.028} $  &  $ 0.27^{+0.25}_{-0.19} $  &  $ 17.8813 \pm 0.00013 $  &  $ 715.2518 \pm 0.005 $  & 41 &  $ 23.0^{+11.0}_{-4.0} $  &  $ 0.263 \pm 0.051 $  \\
38138512 &  $ 1.337 \pm 0.069 $  &  $ 0.52 \pm 0.12 $  &  $ 1559.9513 \pm 0.0022 $  &  $ 2300.0253^{+0.0025}_{-0.0026} $  &  $ 17.8 \pm 1.0 $  &  $ 0.2708^{+0.0073}_{-0.0058} $  &  $ 0.32 \pm 0.2 $  &  $ 18.50185 \pm 8e-05 $  &  $ 740.074 \pm 0.0033 $  & 41 &  $ 21.1^{+6.3}_{-2.2} $  &  $ 0.15^{+0.068}_{-0.009} $  \\
71028120 &  $ 1.375 \pm 0.062 $  &  $ 0.393^{+0.087}_{-0.075} $  &  $ 1445.8159 \pm 0.0042 $  &  $ 2189.9538 \pm 0.0041 $  &  $ 4.74 \pm 0.31 $  &  $ 0.2569^{+0.009}_{-0.0084} $  &  $ 0.38^{+0.22}_{-0.25} $  &  $ 18.60345 \pm 0.00014 $  &  $ 744.1379 \pm 0.0055 $  & 41 &  $ 21.3^{+6.3}_{-2.7} $  &  $ 0.18^{+0.073}_{-0.022} $  \\
124029677 &  $ 1.386 \pm 0.061 $  &  $ 0.53 \pm 0.13 $  &  $ 1486.1214 \pm 0.0015 $  &  $ 2218.0049 \pm 0.0014 $  &  $ 11.35 \pm 0.59 $  &  $ 0.1944^{+0.0059}_{-0.0041} $  &  $ 0.43^{+0.22}_{-0.28} $  &  $ 18.76624^{+6e-05}_{-5e-05} $  &  $ 731.8834 \pm 0.002 $  & 40 &  $ 20.9^{+5.2}_{-2.1} $  &  $ 0.35^{+0.073}_{-0.035} $  \\
366322247 &  $ 2.92^{+0.15}_{-0.15} $  &  $ 0.059^{+0.017}_{-0.014} $  &  $ 1618.2953 \pm 0.0011 $  &  $ 2352.4106 \pm 0.0011 $  &  $ 38.0^{+17.0}_{-10.0} $  &  $ 0.1231 \pm 0.0061 $  &  $ 1.015^{+0.067}_{-0.049} $  &  $ 18.82347 \pm 4e-05 $  &  $ 734.1152 \pm 0.0016 $  & 40 &  $ 21.0^{+5.2}_{-2.2} $  &  $ 0.689^{+0.04}_{-0.021} $  \\
211409161 &  $ 0.783 \pm 0.056 $  &  $ 1.77^{+0.56}_{-0.45} $  &  $ 1335.10057 \pm 0.00077 $  &  $ 2070.36568 \pm 0.00063 $  &  $ 13.1^{+4.5}_{-2.6} $  &  $ 0.0991 \pm 0.0046 $  &  $ 0.943^{+0.077}_{-0.066} $  &  $ 18.85295 \pm 3e-05 $  &  $ 735.2651 \pm 0.001 $  & 40 &  $ 21.0^{+5.3}_{-2.2} $  &  $ 0.269^{+0.08}_{-0.036} $  \\
317923092 &  $ 1.342^{+0.054}_{-0.056} $  &  $ 0.69^{+0.17}_{-0.13} $  &  $ 1479.8227 \pm 0.0092 $  &  $ 2209.4197^{+0.0089}_{-0.0078} $  &  $ 14.1^{+6.7}_{-2.4} $  &  $ 0.494 \pm 0.038 $  &  $ 0.953^{+0.07}_{-0.048} $  &  $ 19.19992 \pm 0.00032 $  &  $ 729.597 \pm 0.012 $  & 39 &  $ 29.0^{+16.0}_{-6.0} $  &  $ 0.856^{+0.018}_{-0.043} $  \\
14445414 &  $ 1.315 \pm 0.067 $  &  $ 0.57^{+0.19}_{-0.13} $  &  $ 1497.5559 \pm 0.0014 $  &  $ 2210.9761 \pm 0.0014 $  &  $ 7.5^{+3.9}_{-1.2} $  &  $ 0.12 \pm 0.013 $  &  $ 0.93^{+0.06}_{-0.18} $  &  $ 19.28163^{+5e-05}_{-6e-05} $  &  $ 713.4202 \pm 0.0019 $  & 38 &  $ 22.3^{+7.4}_{-3.0} $  &  $ 0.316^{+0.034}_{-0.004} $  \\
32179255 &  $ 1.751 \pm 0.08 $  &  $ 0.218^{+0.049}_{-0.04} $  &  $ 1345.8792 \pm 0.0018 $  &  $ 2068.4541 \pm 0.0016 $  &  $ 21.0 \pm 8.0 $  &  $ 0.1565 \pm 0.0062 $  &  $ 0.999^{+0.07}_{-0.045} $  &  $ 20.645 \pm 7e-05 $  &  $ 722.5749 \pm 0.0024 $  & 36 &  $ 22.6^{+6.3}_{-1.9} $  &  $ 0.196^{+0.091}_{-0.027} $  \\
123763494 &  $ 1.21 \pm 0.063 $  &  $ 0.6^{+0.16}_{-0.13} $  &  $ 1486.92889 \pm 0.00089 $  &  $ 2209.76761^{+0.00073}_{-0.00087} $  &  $ 19.8^{+7.1}_{-4.5} $  &  $ 0.1031 \pm 0.0047 $  &  $ 0.97^{+0.076}_{-0.062} $  &  $ 19.53618 \pm 3e-05 $  &  $ 722.8387 \pm 0.0012 $  & 38 &  $ 21.9^{+5.9}_{-2.4} $  &  $ 0.515^{+0.064}_{-0.033} $  \\
13713700 &  $ 0.97 \pm 0.047 $  &  $ 1.17^{+0.28}_{-0.23} $  &  $ 1536.982 \pm 0.0017 $  &  $ 2245.8286 \pm 0.0018 $  &  $ 8.3 \pm 1.0 $  &  $ 0.144 \pm 0.011 $  &  $ 0.79^{+0.11}_{-0.28} $  &  $ 19.69018^{+7e-05}_{-6e-05} $  &  $ 708.8466^{+0.0025}_{-0.0024} $  & 37 &  $ 22.9^{+8.0}_{-3.2} $  &  $ 0.285^{+0.042}_{-0.009} $  \\
300394149 &  $ 1.426^{+0.065}_{-0.067} $  &  $ 0.364^{+0.092}_{-0.073} $  &  $ 1576.8835^{+0.0044}_{-0.0046} $  &  $ 2325.4236 \pm 0.0041 $  &  $ 6.46 \pm 0.34 $  &  $ 0.55 \pm 0.01 $  &  $ 0.27 \pm 0.22 $  &  $ 19.69843 \pm 0.00016 $  &  $ 748.5402 \pm 0.0062 $  & 39 &  $ 26.0^{+16.0}_{-6.0} $  &  $ 0.58^{+0.05}_{-0.11} $  \\
1504460 &  $ 1.504 \pm 0.068 $  &  $ 0.374^{+0.098}_{-0.08} $  &  $ 1528.397 \pm 0.0022 $  &  $ 2261.1202 \pm 0.0022 $  &  $ 9.6 \pm 1.0 $  &  $ 0.167^{+0.017}_{-0.012} $  &  $ 0.78^{+0.12}_{-0.37} $  &  $ 19.80333^{+8e-05}_{-9e-05} $  &  $ 732.7232 \pm 0.0031 $  & 24 &  $ 20.0^{+19.0}_{-1.0} $  &  $ 0.37^{+0.13}_{-0.0} $  \\
13072758 &  $ 1.43 \pm 0.068 $  &  $ 0.38 \pm 0.1 $  &  $ 1455.5937 \pm 0.0044 $  &  $ 2193.2135 \pm 0.0037 $  &  $ 11.78^{+0.67}_{-0.65} $  &  $ 0.384 \pm 0.01 $  &  $ 0.31 \pm 0.22 $  &  $ 19.93567 \pm 0.00015 $  &  $ 737.6197 \pm 0.0057 $  & 38 &  $ 26.0 \pm 10.0 $  &  $ 0.276^{+0.075}_{-0.087} $  \\
107113345 &  $ 1.313 \pm 0.058 $  &  $ 0.65^{+0.18}_{-0.14} $  &  $ 1576.32835^{+0.00051}_{-0.00056} $  &  $ 2317.29686^{+0.00055}_{-0.00055} $  &  $ 9.2^{+5.1}_{-2.3} $  &  $ 0.0968 \pm 0.0081 $  &  $ 0.976 \pm 0.048 $  &  $ 20.02618 \pm 2e-05 $  &  $ 740.96854 \pm 0.00077 $  & 38 &  $ 22.5^{+6.0}_{-2.4} $  &  $ 0.243^{+0.067}_{-0.019} $  \\
437293313 &  $ 0.937 \pm 0.049 $  &  $ 1.08^{+0.3}_{-0.22} $  &  $ 1578.4471 \pm 0.0042 $  &  $ 2328.0893 \pm 0.004 $  &  $ 8.57^{+0.56}_{-0.52} $  &  $ 0.2639^{+0.0096}_{-0.009} $  &  $ 0.25 \pm 0.2 $  &  $ 20.2606 \pm 0.00015 $  &  $ 749.6422 \pm 0.0056 $  & 38 &  $ 27.0 \pm 9.0 $  &  $ 0.233^{+0.066}_{-0.061} $  \\
70561926 &  $ 1.355 \pm 0.062 $  &  $ 0.58 \pm 0.14 $  &  $ 1523.06374 \pm 0.00068 $  &  $ 2275.36045 \pm 0.00059 $  &  $ 17.51 \pm 0.82 $  &  $ 0.2499 \pm 0.0018 $  &  $ 0.15 \pm 0.12 $  &  $ 20.33234^{+3e-05}_{-2e-05} $  &  $ 752.29671 \pm 0.00091 $  & 38 &  $ 22.1^{+5.7}_{-1.8} $  &  $ 0.226^{+0.09}_{-0.032} $  \\
39167176 &  $ 1.558 \pm 0.094 $  &  $ 0.51 \pm 0.13 $  &  $ 1470.6242 \pm 0.0033 $  &  $ 2211.4275 \pm 0.0037 $  &  $ 18.8^{+8.9}_{-2.9} $  &  $ 0.274 \pm 0.014 $  &  $ 0.947^{+0.081}_{-0.044} $  &  $ 20.57787 \pm 0.00014 $  &  $ 740.8033 \pm 0.005 $  & 37 &  $ 26.0^{+20.0}_{-5.0} $  &  $ 0.52 \pm 0.1 $  \\
381553868 &  $ 1.6 \pm 0.093 $  &  $ 0.33 \pm 0.09 $  &  $ 1677.3243^{+0.0034}_{-0.0036} $  &  $ 2367.5791 \pm 0.0032 $  &  $ 12.41 \pm 0.84 $  &  $ 0.2748^{+0.0093}_{-0.0072} $  &  $ 0.39^{+0.22}_{-0.26} $  &  $ 20.91681 \pm 0.00014 $  &  $ 690.2549 \pm 0.0047 $  & 33 &  $ 23.8^{+6.2}_{-2.9} $  &  $ 0.225^{+0.073}_{-0.032} $  \\
296737508 &  $ 1.271 \pm 0.069 $  &  $ 0.51 \pm 0.12 $  &  $ 1538.0031 \pm 0.0014 $  &  $ 2272.004 \pm 0.0023 $  &  $ 5.88 \pm 0.36 $  &  $ 0.2185^{+0.0049}_{-0.0044} $  &  $ 0.6^{+0.12}_{-0.26} $  &  $ 20.97145^{+8e-05}_{-7e-05} $  &  $ 734.0009 \pm 0.0027 $  & 36 &  $ 23.7^{+6.9}_{-2.7} $  &  $ 0.203^{+0.063}_{-0.015} $  \\
2669681 &  $ 1.88 \pm 0.12 $  &  $ 0.126^{+0.038}_{-0.029} $  &  $ 1676.7343 \pm 0.0033 $  &  $ 2044.4557 \pm 0.003 $  &  $ 17.0 \pm 1.2 $  &  $ 0.399 \pm 0.011 $  &  $ 0.66^{+0.09}_{-0.24} $  &  $ 21.63067^{+0.00026}_{-0.00025} $  &  $ 367.7214 \pm 0.0044 $  & 18 &  $ 24.5^{+8.9}_{-2.9} $  &  $ 0.187^{+0.018}_{-0.008} $  \\
157119927 &  $ 1.036 \pm 0.054 $  &  $ 0.96 \pm 0.2 $  &  $ 1591.6217 \pm 0.0011 $  &  $ 2291.006 \pm 0.001 $  &  $ 13.4^{+5.9}_{-3.1} $  &  $ 0.1119^{+0.0069}_{-0.0062} $  &  $ 0.983^{+0.071}_{-0.048} $  &  $ 21.19346^{+5e-05}_{-4e-05} $  &  $ 699.3843 \pm 0.0014 $  & 34 &  $ 24.1^{+6.3}_{-2.9} $  &  $ 0.176^{+0.075}_{-0.025} $  \\
118339710 &  $ 1.566 \pm 0.07 $  &  $ 0.291^{+0.075}_{-0.063} $  &  $ 1525.6471 \pm 0.0022 $  &  $ 2249.5472 \pm 0.0019 $  &  $ 10.64^{+0.65}_{-0.61} $  &  $ 0.372 \pm 0.011 $  &  $ 0.48 \pm 0.29 $  &  $ 21.29118^{+8e-05}_{-9e-05} $  &  $ 723.9001 \pm 0.0029 $  & 26 &  $ 33.0 \pm 12.0 $  &  $ 0.231^{+0.081}_{-0.013} $  \\
207783865 &  $ 1.039 \pm 0.051 $  &  $ 1.04^{+0.28}_{-0.21} $  &  $ 1608.93658 \pm 0.00044 $  &  $ 2354.11347 \pm 0.00034 $  &  $ 15.26 \pm 0.79 $  &  $ 0.0837 \pm 0.0021 $  &  $ 0.801^{+0.024}_{-0.035} $  &  $ 21.29077^{+1e-05}_{-2e-05} $  &  $ 745.1769^{+0.00053}_{-0.00055} $  & 36 &  $ 23.3^{+6.5}_{-2.0} $  &  $ 0.722^{+0.041}_{-0.016} $  \\
176518126 &  $ 1.36 \pm 0.18 $  &  $ 0.71^{+0.38}_{-0.25} $  &  $ 1489.0554 \pm 0.0027 $  &  $ 2219.5376 \pm 0.0018 $  &  $ 8.4 \pm 1.1 $  &  $ 0.2361^{+0.0051}_{-0.0042} $  &  $ 0.31 \pm 0.23 $  &  $ 21.48477 \pm 0.0001 $  &  $ 730.4822 \pm 0.0033 $  & 35 &  $ 25.2^{+6.6}_{-3.7} $  &  $ 0.2^{+0.047}_{-0.013} $  \\
290165539 &  $ 1.332 \pm 0.071 $  &  $ 0.42 \pm 0.1 $  &  $ 1332.7557 \pm 0.003 $  &  $ 2067.9702 \pm 0.0043 $  &  $ 23.4^{+6.3}_{-3.4} $  &  $ 0.47 \pm 0.011 $  &  $ 0.95^{+0.066}_{-0.046} $  &  $ 21.62396 \pm 0.00015 $  &  $ 735.2146 \pm 0.0052 $  & 35 &  $ 27.0^{+19.0}_{-5.0} $  &  $ 0.723^{+0.03}_{-0.091} $  \\
339399841 &  $ 1.545 \pm 0.081 $  &  $ 0.277^{+0.072}_{-0.057} $  &  $ 1662.1116^{+0.0046}_{-0.0041} $  &  $ 2043.5951 \pm 0.005 $  &  $ 13.0^{+1.7}_{-1.1} $  &  $ 0.256^{+0.035}_{-0.018} $  &  $ 0.73^{+0.15}_{-0.34} $  &  $ 22.4402 \pm 0.00038 $  &  $ 381.4834^{+0.0065}_{-0.0065} $  & 18 &  $ 25.4^{+9.2}_{-4.2} $  &  $ 0.31^{+0.036}_{-0.011} $  \\
237605045 &  $ 2.92 \pm 0.16 $  &  $ 0.064 \pm 0.019 $  &  $ 1489.0429^{+0.0014}_{-0.0015} $  &  $ 2210.2969 \pm 0.0014 $  &  $ 42.0^{+18.0}_{-10.0} $  &  $ 0.1739^{+0.0048}_{-0.0041} $  &  $ 1.002^{+0.076}_{-0.054} $  &  $ 21.85619^{+5e-05}_{-6e-05} $  &  $ 721.2541 \pm 0.0019 $  & 34 &  $ 24.0^{+6.0}_{-2.2} $  &  $ 0.565^{+0.054}_{-0.025} $  \\
442893494 &  $ 1.393 \pm 0.064 $  &  $ 0.44 \pm 0.11 $  &  $ 1472.659 \pm 0.0038 $  &  $ 2194.3845^{+0.004}_{-0.0047} $  &  $ 11.55^{+0.67}_{-0.63} $  &  $ 0.308 \pm 0.01 $  &  $ 0.34^{+0.25}_{-0.23} $  &  $ 21.87047 \pm 0.00017 $  &  $ 721.7255^{+0.0054}_{-0.0058} $  & 22 &  $ 36.0 \pm 12.0 $  &  $ 0.201^{+0.054}_{-0.006} $  \\
292719109 &  $ 2.08 \pm 0.1 $  &  $ 0.144^{+0.039}_{-0.031} $  &  $ 1499.7023 \pm 0.0022 $  &  $ 2222.3189 \pm 0.0024 $  &  $ 11.07 \pm 0.59 $  &  $ 0.3704^{+0.0054}_{-0.0045} $  &  $ 0.34 \pm 0.23 $  &  $ 21.89747 \pm 0.0001 $  &  $ 722.6166 \pm 0.0032 $  & 34 &  $ 24.1^{+7.3}_{-2.2} $  &  $ 0.202^{+0.087}_{-0.025} $  \\
9844069 &  $ 1.607 \pm 0.087 $  &  $ 0.25^{+0.065}_{-0.052} $  &  $ 1431.1663 \pm 0.0038 $  &  $ 2148.9232 \pm 0.0034 $  &  $ 18.9 \pm 1.4 $  &  $ 0.301^{+0.015}_{-0.013} $  &  $ 0.62^{+0.12}_{-0.3} $  &  $ 22.42991 \pm 0.00016 $  &  $ 717.7571 \pm 0.0049 $  & 33 &  $ 25.6^{+7.0}_{-3.2} $  &  $ 0.218^{+0.063}_{-0.022} $  \\
275878706 &  $ 0.933 \pm 0.063 $  &  $ 0.97^{+0.33}_{-0.24} $  &  $ 1621.0799 \pm 0.0027 $  &  $ 2341.7827 \pm 0.0028 $  &  $ 8.1^{+3.1}_{-1.3} $  &  $ 0.172 \pm 0.017 $  &  $ 0.88^{+0.09}_{-0.21} $  &  $ 22.52196 \pm 0.00012 $  &  $ 720.7028 \pm 0.0039 $  & 33 &  $ 27.0^{+11.0}_{-4.0} $  &  $ 0.316^{+0.016}_{-0.009} $  \\
77437543 &  $ 1.171 \pm 0.062 $  &  $ 0.57 \pm 0.13 $  &  $ 1456.7034 \pm 0.0017 $  &  $ 2180.6921 \pm 0.0014 $  &  $ 10.98^{+0.66}_{-0.63} $  &  $ 0.3221^{+0.0063}_{-0.0046} $  &  $ 0.31 \pm 0.22 $  &  $ 22.62465 \pm 7e-05 $  &  $ 723.9887 \pm 0.0022 $  & 22 &  $ 38.0^{+14.0}_{-15.0} $  &  $ 0.246^{+0.03}_{-0.088} $  \\
159490807 &  $ 1.693^{+0.083}_{-0.085} $  &  $ 0.256^{+0.076}_{-0.056} $  &  $ 1606.226 \pm 0.0023 $  &  $ 2355.9376 \pm 0.0021 $  &  $ 15.4^{+4.7}_{-1.6} $  &  $ 0.2163 \pm 0.0082 $  &  $ 0.938^{+0.048}_{-0.025} $  &  $ 22.71853^{+0.0001}_{-9e-05} $  &  $ 749.7116 \pm 0.003 $  & 34 &  $ 29.0 \pm 8.0 $  &  $ 0.204^{+0.039}_{-0.027} $  \\
289840544 &  $ 1.75 \pm 0.11 $  &  $ 0.223^{+0.062}_{-0.049} $  &  $ 1331.2898 \pm 0.0014 $  &  $ 2083.2879 \pm 0.0015 $  &  $ 14.0^{+9.1}_{-3.6} $  &  $ 0.135 \pm 0.011 $  &  $ 0.984^{+0.063}_{-0.045} $  &  $ 22.78782^{+7e-05}_{-6e-05} $  &  $ 751.9982 \pm 0.002 $  & 34 &  $ 25.1^{+6.3}_{-2.3} $  &  $ 0.284^{+0.073}_{-0.027} $  \\
332697924 &  $ 1.315 \pm 0.06 $  &  $ 0.54 \pm 0.12 $  &  $ 1445.7501^{+0.0055}_{-0.0051} $  &  $ 2178.2146 \pm 0.005 $  &  $ 4.69 \pm 0.33 $  &  $ 0.256 \pm 0.01 $  &  $ 0.34 \pm 0.23 $  &  $ 22.88951 \pm 0.00023 $  &  $ 732.4644^{+0.0076}_{-0.0074} $  & 33 &  $ 26.2^{+7.1}_{-3.3} $  &  $ 0.173^{+0.058}_{-0.013} $  \\
242241304 &  $ 1.138^{+0.055}_{-0.057} $  &  $ 0.69^{+0.16}_{-0.13} $  &  $ 1623.0701 \pm 0.0028 $  &  $ 2345.3738 \pm 0.0026 $  &  $ 9.7 \pm 1.0 $  &  $ 0.178 \pm 0.012 $  &  $ 0.855^{+0.061}_{-0.071} $  &  $ 23.30012 \pm 0.00012 $  &  $ 722.3037 \pm 0.0037 $  & 32 &  $ 28.0^{+10.0}_{-4.0} $  &  $ 0.228^{+0.018}_{-0.006} $  \\
412386707 &  $ 1.96 \pm 0.092 $  &  $ 0.18^{+0.046}_{-0.039} $  &  $ 1493.9545^{+0.0025}_{-0.0026} $  &  $ 2240.5723^{+0.0025}_{-0.0024} $  &  $ 12.37 \pm 0.81 $  &  $ 0.225 \pm 0.01 $  &  $ 0.65^{+0.15}_{-0.38} $  &  $ 23.33181 \pm 0.00011 $  &  $ 746.6178^{+0.0037}_{-0.0035} $  & 33 &  $ 25.7^{+6.7}_{-2.4} $  &  $ 0.468^{+0.065}_{-0.029} $  \\
188620407 &  $ 1.306 \pm 0.064 $  &  $ 0.54 \pm 0.13 $  &  $ 1375.487 \pm 0.0026 $  &  $ 2461.7057 \pm 0.0024 $  &  $ 9.65 \pm 0.54 $  &  $ 0.2623^{+0.0073}_{-0.0059} $  &  $ 0.4^{+0.22}_{-0.27} $  &  $ 24.1382 \pm 8e-05 $  &  $ 1086.2188 \pm 0.0036 $  & 35 &  $ 28.0 \pm 10.0 $  &  $ 0.18^{+0.11}_{-0.02} $  \\
457649900 &  $ 2.112^{+0.096}_{-0.092} $  &  $ 0.137^{+0.042}_{-0.033} $  &  $ 1606.9707^{+0.0059}_{-0.0053} $  &  $ 2355.7959 \pm 0.0051 $  &  $ 18.0^{+9.8}_{-3.9} $  &  $ 0.283 \pm 0.019 $  &  $ 0.986^{+0.058}_{-0.033} $  &  $ 23.40078 \pm 0.00023 $  &  $ 748.825^{+0.0075}_{-0.0075} $  & 33 &  $ 30.0^{+20.0}_{-6.0} $  &  $ 0.4 \pm 0.1 $  \\
404518509 &  $ 1.035 \pm 0.05 $  &  $ 0.96 \pm 0.22 $  &  $ 1431.2685 \pm 0.0031 $  &  $ 2134.8844 \pm 0.0025 $  &  $ 2.72 \pm 0.17 $  &  $ 0.2059 \pm 0.006 $  &  $ 0.35^{+0.28}_{-0.24} $  &  $ 23.45386 \pm 0.00013 $  &  $ 703.6158 \pm 0.004 $  & 18 &  $ 23.0^{+12.0}_{-1.0} $  &  $ 0.183^{+0.088}_{-0.004} $  \\
199738560 &  $ 1.91 \pm 0.4 $  &  $ 0.1^{+0.092}_{-0.046} $  &  $ 1390.8573 \pm 0.0053 $  &  $ 2121.9547 \pm 0.0053 $  &  $ 25.0 \pm 5.8 $  &  $ 0.403 \pm 0.021 $  &  $ 0.838^{+0.046}_{-0.083} $  &  $ 38.4788 \pm 0.00038 $  &  $ 731.0972 \pm 0.0073 $  & 20 &  $ 41.0^{+12.0}_{-18.0} $  &  $ 0.261^{+0.032}_{-0.009} $  \\
333736132 &  $ 0.755^{+0.056}_{-0.053} $  &  $ 2.03^{+0.75}_{-0.54} $  &  $ 1551.55314 \pm 0.00099 $  &  $ 2283.54678^{+0.00086}_{-0.00078} $  &  $ 10.25^{+0.87}_{-0.82} $  &  $ 0.1223 \pm 0.0044 $  &  $ 0.751^{+0.045}_{-0.091} $  &  $ 23.6127 \pm 4e-05 $  &  $ 731.9937 \pm 0.0013 $  & 32 &  $ 26.1^{+7.1}_{-2.5} $  &  $ 0.324^{+0.083}_{-0.036} $  \\
306249066 &  $ 1.136^{+0.056}_{-0.053} $  &  $ 0.77^{+0.19}_{-0.15} $  &  $ 1593.9762 \pm 0.0016 $  &  $ 2326.5146 \pm 0.0014 $  &  $ 11.09 \pm 0.61 $  &  $ 0.1628 \pm 0.0054 $  &  $ 0.867 \pm 0.021 $  &  $ 23.63027 \pm 7e-05 $  &  $ 732.5384 \pm 0.0021 $  & 32 &  $ 27.1^{+7.8}_{-3.5} $  &  $ 0.144^{+0.057}_{-0.005} $  \\
313671132 &  $ 1.219 \pm 0.061 $  &  $ 0.57^{+0.15}_{-0.12} $  &  $ 1604.3534 \pm 0.003 $  &  $ 2337.7277 \pm 0.0032 $  &  $ 7.78^{+0.67}_{-0.62} $  &  $ 0.224 \pm 0.02 $  &  $ 0.81^{+0.08}_{-0.22} $  &  $ 23.65724 \pm 0.00014 $  &  $ 733.3743 \pm 0.0043 $  & 32 &  $ 28.0^{+13.0}_{-5.0} $  &  $ 0.311 \pm 0.011 $  \\
265465927 &  $ 1.161 \pm 0.057 $  &  $ 0.72^{+0.17}_{-0.13} $  &  $ 1342.6468 \pm 0.0022 $  &  $ 2058.6086 \pm 0.002 $  &  $ 11.73 \pm 0.63 $  &  $ 0.263^{+0.0055}_{-0.0046} $  &  $ 0.27 \pm 0.19 $  &  $ 23.86539 \pm 0.0001 $  &  $ 715.9618 \pm 0.003 $  & 31 &  $ 27.5^{+8.3}_{-3.7} $  &  $ 0.143^{+0.061}_{-0.006} $  \\
42428568 &  $ 2.15 \pm 0.12 $  &  $ 0.128^{+0.042}_{-0.033} $  &  $ 1475.6901^{+0.0046}_{-0.0043} $  &  $ 2224.326 \pm 0.0039 $  &  $ 24.0^{+11.0}_{-5.0} $  &  $ 0.393 \pm 0.012 $  &  $ 0.981^{+0.066}_{-0.038} $  &  $ 24.14954 \pm 0.0002 $  &  $ 748.6358 \pm 0.0062 $  & 32 &  $ 31.0^{+22.0}_{-6.0} $  &  $ 0.52 \pm 0.1 $  \\
466206508 &  $ 1.269 \pm 0.071 $  &  $ 0.43 \pm 0.1 $  &  $ 1679.3454 \pm 0.0019 $  &  $ 2054.9734 \pm 0.0018 $  &  $ 13.55 \pm 0.82 $  &  $ 0.3625^{+0.0069}_{-0.0057} $  &  $ 0.37 \pm 0.2 $  &  $ 25.04186 \pm 0.00018 $  &  $ 375.628 \pm 0.0026 $  & 16 &  $ 31.0^{+16.0}_{-6.0} $  &  $ 0.209^{+0.042}_{-0.051} $  \\
67599025 &  $ 0.775 \pm 0.052 $  &  $ 1.85^{+0.56}_{-0.44} $  &  $ 1404.0208 \pm 0.0014 $  &  $ 2138.8254 \pm 0.0014 $  &  $ 6.86 \pm 0.57 $  &  $ 0.1316^{+0.0067}_{-0.006} $  &  $ 0.62^{+0.13}_{-0.35} $  &  $ 24.49349^{+6e-05}_{-7e-05} $  &  $ 734.8047 \pm 0.0019 $  & 31 &  $ 27.2^{+7.8}_{-2.7} $  &  $ 0.343^{+0.079}_{-0.031} $  \\
101824521 &  $ 1.235 \pm 0.069 $  &  $ 0.47 \pm 0.12 $  &  $ 1620.3536^{+0.0046}_{-0.0043} $  &  $ 2331.5276 \pm 0.0026 $  &  $ 12.17 \pm 0.72 $  &  $ 0.3574 \pm 0.0062 $  &  $ 0.18^{+0.18}_{-0.13} $  &  $ 24.52324 \pm 0.00018 $  &  $ 711.174 \pm 0.0052 $  & 30 &  $ 31.0 \pm 10.0 $  &  $ 0.187^{+0.055}_{-0.035} $  \\
256912435 &  $ 1.191 \pm 0.059 $  &  $ 0.65^{+0.17}_{-0.13} $  &  $ 1623.43765 \pm 0.0008 $  &  $ 2338.70956 \pm 0.00077 $  &  $ 25.5^{+4.6}_{-3.8} $  &  $ 0.1099 \pm 0.0034 $  &  $ 0.95 \pm 0.051 $  &  $ 24.66455 \pm 4e-05 $  &  $ 715.2719 \pm 0.0011 $  & 30 &  $ 27.5^{+6.6}_{-2.8} $  &  $ 0.628^{+0.046}_{-0.026} $  \\
142278054 &  $ 2.39 \pm 0.12 $  &  $ 0.105^{+0.029}_{-0.023} $  &  $ 1595.0238 \pm 0.0029 $  &  $ 2310.3521^{+0.0023}_{-0.0025} $  &  $ 11.49^{+0.96}_{-0.91} $  &  $ 0.212 \pm 0.012 $  &  $ 0.79^{+0.11}_{-0.38} $  &  $ 24.66649 \pm 0.00013 $  &  $ 715.3282 \pm 0.0038 $  & 30 &  $ 27.5^{+6.6}_{-2.8} $  &  $ 0.52^{+0.055}_{-0.029} $  \\
268534931 &  $ 0.776 \pm 0.044 $  &  $ 1.72^{+0.53}_{-0.4} $  &  $ 1398.2954 \pm 0.0039 $  &  $ 2139.099^{+0.0034}_{-0.0036} $  &  $ 6.12 \pm 0.39 $  &  $ 0.305 \pm 0.009 $  &  $ 0.29 \pm 0.23 $  &  $ 24.69345 \pm 0.00018 $  &  $ 740.8036^{+0.0054}_{-0.0055} $  & 31 &  $ 32.0^{+25.0}_{-7.0} $  &  $ 0.46^{+0.06}_{-0.16} $  \\
161169240 &  $ 1.192 \pm 0.06 $  &  $ 0.6 \pm 0.13 $  &  $ 1328.2601 \pm 0.0024 $  &  $ 2083.315^{+0.0025}_{-0.0025} $  &  $ 12.19^{+0.77}_{-0.73} $  &  $ 0.303 \pm 0.009 $  &  $ 0.47^{+0.21}_{-0.29} $  &  $ 26.03638 \pm 0.00012 $  &  $ 755.055^{+0.0035}_{-0.0034} $  & 30 &  $ 31.0^{+13.0}_{-4.0} $  &  $ 0.206^{+0.03}_{-0.015} $  \\
439491923 &  $ 1.257^{+0.065}_{-0.065} $  &  $ 0.53 \pm 0.13 $  &  $ 1405.412 \pm 0.0046 $  &  $ 2116.7942 \pm 0.0038 $  &  $ 13.9 \pm 1.3 $  &  $ 0.286^{+0.027}_{-0.017} $  &  $ 0.7^{+0.14}_{-0.3} $  &  $ 26.34748 \pm 0.00023 $  &  $ 711.3821 \pm 0.0062 $  & 28 &  $ 31.0^{+14.0}_{-5.0} $  &  $ 0.27 \pm 0.011 $  \\
218977148 &  $ 1.612 \pm 0.092 $  &  $ 0.296^{+0.082}_{-0.066} $  &  $ 1355.4698 \pm 0.006 $  &  $ 2090.0979 \pm 0.0053 $  &  $ 11.9 \pm 0.82 $  &  $ 0.326 \pm 0.013 $  &  $ 0.4^{+0.22}_{-0.26} $  &  $ 27.20845 \pm 0.00032 $  &  $ 734.6281 \pm 0.0087 $  & 28 &  $ 30.6^{+8.1}_{-3.4} $  &  $ 0.193^{+0.063}_{-0.02} $  \\
304339227 &  $ 1.125 \pm 0.049 $  &  $ 0.78 \pm 0.17 $  &  $ 1673.3376 \pm 0.0038 $  &  $ 2388.0219 \pm 0.0041 $  &  $ 2.71 \pm 0.17 $  &  $ 0.238 \pm 0.009 $  &  $ 0.34 \pm 0.24 $  &  $ 27.48785 \pm 0.00021 $  &  $ 714.6842^{+0.0057}_{-0.0054} $  & 27 &  $ 31.1^{+8.6}_{-3.6} $  &  $ 0.175^{+0.058}_{-0.012} $  \\
265466589 &  $ 1.029 \pm 0.05 $  &  $ 1.03^{+0.28}_{-0.21} $  &  $ 1352.5249 \pm 0.0024 $  &  $ 2037.8661 \pm 0.0023 $  &  $ 8.68 \pm 0.58 $  &  $ 0.1785^{+0.0087}_{-0.0071} $  &  $ 0.49^{+0.21}_{-0.31} $  &  $ 28.55588 \pm 0.00014 $  &  $ 685.3412 \pm 0.0034 $  & 25 &  $ 31.2^{+9.2}_{-3.7} $  &  $ 0.33^{+0.08}_{-0.036} $  \\
220622886 &  $ 2.56 \pm 0.13 $  &  $ 0.066^{+0.017}_{-0.014} $  &  $ 1479.5256 \pm 0.003 $  &  $ 2204.5847 \pm 0.0029 $  &  $ 28.0^{+16.0}_{-8.0} $  &  $ 0.227 \pm 0.016 $  &  $ 0.994^{+0.071}_{-0.048} $  &  $ 42.65054^{+0.00025}_{-0.00024} $  &  $ 725.0591 \pm 0.0042 $  & 18 &  $ 29.0^{+23.0}_{-0.0} $  &  $ 0.3^{+0.19}_{-0.0} $  \\
156716001 &  $ 1.086 \pm 0.048 $  &  $ 0.83 \pm 0.2 $  &  $ 1485.4058 \pm 0.0032 $  &  $ 2224.5177 \pm 0.0034 $  &  $ 5.97 \pm 0.3 $  &  $ 0.3643^{+0.0087}_{-0.0066} $  &  $ 0.28 \pm 0.22 $  &  $ 33.596 \pm 0.00022 $  &  $ 739.112 \pm 0.0048 $  & 23 &  $ 43.0^{+30.0}_{-10.0} $  &  $ 0.33 \pm 0.1 $  \\
81089255 &  $ 1.429 \pm 0.051 $  &  $ 0.62 \pm 0.13 $  &  $ 1509.9452 \pm 0.0027 $  &  $ 2260.2072 \pm 0.0024 $  &  $ 12.19 \pm 0.69 $  &  $ 0.191 \pm 0.01 $  &  $ 0.76^{+0.07}_{-0.26} $  &  $ 34.10282 \pm 0.00016 $  &  $ 750.262 \pm 0.0036 $  & 23 &  $ 37.5^{+9.4}_{-4.9} $  &  $ 0.316^{+0.07}_{-0.037} $  \\
52195587 &  $ 1.2 \pm 0.056 $  &  $ 0.56 \pm 0.11 $  &  $ 1350.2761 \pm 0.004 $  &  $ 2107.6102 \pm 0.0041 $  &  $ 9.28 \pm 0.52 $  &  $ 0.348 \pm 0.01 $  &  $ 0.29 \pm 0.22 $  &  $ 34.42428 \pm 0.00026 $  &  $ 757.3342 \pm 0.0057 $  & 18 &  $ 50.0 \pm 17.0 $  &  $ 0.188^{+0.051}_{-0.028} $  \\
140215502 &  $ 0.928 \pm 0.046 $  &  $ 1.1^{+0.32}_{-0.25} $  &  $ 1460.5483^{+0.0057}_{-0.0041} $  &  $ 2194.4407^{+0.0027}_{-0.0024} $  &  $ 5.87^{+0.37}_{-0.33} $  &  $ 0.2912^{+0.0076}_{-0.0067} $  &  $ 0.27^{+0.28}_{-0.19} $  &  $ 34.94726^{+0.00023}_{-0.0003} $  &  $ 733.8924^{+0.005}_{-0.0062} $  & 22 &  $ 43.0^{+18.0}_{-8.0} $  &  $ 0.225^{+0.054}_{-0.039} $  \\
157698565 &  $ 1.07 \pm 0.05 $  &  $ 0.81 \pm 0.19 $  &  $ 1494.5801 \pm 0.0013 $  &  $ 2234.1134 \pm 0.0012 $  &  $ 11.66 \pm 0.59 $  &  $ 0.269 \pm 0.0051 $  &  $ 0.827^{+0.025}_{-0.041} $  &  $ 35.21588^{+8e-05}_{-9e-05} $  &  $ 739.5334 \pm 0.0017 $  & 22 &  $ 46.0^{+28.0}_{-11.0} $  &  $ 0.3 \pm 0.09 $  \\
66439839 &  $ 1.027 \pm 0.048 $  &  $ 1.07^{+0.26}_{-0.22} $  &  $ 1386.34414 \pm 0.00076 $  &  $ 2137.03207 \pm 0.0008 $  &  $ 9.1^{+2.8}_{-1.0} $  &  $ 0.108 \pm 0.013 $  &  $ 0.87^{+0.09}_{-0.29} $  &  $ 37.5344^{+5e-05}_{-6e-05} $  &  $ 750.6879 \pm 0.0011 $  & 17 &  $ 38.0^{+20.0}_{-2.0} $  &  $ 0.51^{+0.11}_{-0.01} $  \\
153838604 &  $ 0.91^{+0.042}_{-0.046} $  &  $ 1.49^{+0.37}_{-0.3} $  &  $ 1447.1024 \pm 0.001 $  &  $ 2176.13855^{+0.00098}_{-0.00086} $  &  $ 17.1^{+4.7}_{-3.3} $  &  $ 0.1086 \pm 0.005 $  &  $ 0.961^{+0.068}_{-0.062} $  &  $ 38.37032^{+8e-05}_{-7e-05} $  &  $ 729.0362 \pm 0.0015 $  & 20 &  $ 41.0^{+12.0}_{-4.0} $  &  $ 0.469^{+0.072}_{-0.033} $  \\
215402824 &  $ 1.326 \pm 0.062 $  &  $ 0.55 \pm 0.13 $  &  $ 1413.62658^{+0.00055}_{-0.00056} $  &  $ 2169.042 \pm 0.0006 $  &  $ 16.0^{+10.0}_{-3.0} $  &  $ 0.098 \pm 0.01 $  &  $ 0.93^{+0.11}_{-0.22} $  &  $ 41.96752^{+5e-05}_{-4e-05} $  &  $ 755.41544^{+0.00085}_{-0.00082} $  & 16 &  $ 42.0^{+21.0}_{-2.0} $  &  $ 0.723^{+0.064}_{-0.01} $  \\
394340183 &  $ 1.035 \pm 0.051 $  &  $ 1.03^{+0.29}_{-0.22} $  &  $ 1664.8425 \pm 0.0013 $  &  $ 2389.114 \pm 0.0016 $  &  $ 10.95 \pm 0.57 $  &  $ 0.3512^{+0.0052}_{-0.0042} $  &  $ 0.32 \pm 0.2 $  &  $ 60.35596 \pm 0.00018 $  &  $ 724.2715 \pm 0.0021 $  & 10 &  $ 72.0^{+18.0}_{-30.0} $  &  $ 0.22^{+0.11}_{-0.04} $  \\
393229954 &  $ 0.904^{+0.043}_{-0.045} $  &  $ 1.44 \pm 0.31 $  &  $ 1446.7995 \pm 0.0011 $  &  $ 2204.5516 \pm 0.0011 $  &  $ 9.3^{+4.1}_{-1.2} $  &  $ 0.116 \pm 0.011 $  &  $ 0.907^{+0.082}_{-0.098} $  &  $ 75.77521 \pm 0.00015 $  &  $ 757.7521^{+0.0015}_{-0.0015} $  & 11 &  $ 45.0^{+31.0}_{-0.0} $  &  $ 0.37^{+0.16}_{-0.0} $  \\
100776118 &  $ 1.248 \pm 0.056 $  &  $ 0.62^{+0.18}_{-0.14} $  &  $ 1472.8146 \pm 0.0027 $  &  $ 2219.6695 \pm 0.0024 $  &  $ 16.37^{+0.73}_{-0.78} $  &  $ 0.9416^{+0.0099}_{-0.0093} $  &  $ 0.844 \pm 0.011 $  &  $ 49.79032 \pm 0.00023 $  &  $ 746.8549^{+0.0036}_{-0.0035} $  & 16 &  $ 62.0^{+31.0}_{-12.0} $  &  $ 0.877^{+0.016}_{-0.034} $  \\
145913596 &  $ 1.453 \pm 0.069 $  &  $ 0.42 \pm 0.11 $  &  $ 1539.5146^{+0.0057}_{-0.0053} $  &  $ 2242.6934^{+0.0078}_{-0.0073} $  &  $ 6.9^{+2.7}_{-1.1} $  &  $ 0.277^{+0.026}_{-0.022} $  &  $ 0.91^{+0.07}_{-0.32} $  &  $ 54.09067 \pm 0.00071 $  &  $ 703.1787 \pm 0.0093 $  & 14 &  $ 59.0^{+29.0}_{-8.0} $  &  $ 0.4239 \pm 0.0059 $  \\
279727635 &  $ 1.046 \pm 0.052 $  &  $ 0.88 \pm 0.21 $  &  $ 1343.2266 \pm 0.0041 $  &  $ 2124.6305 \pm 0.0038 $  &  $ 10.5^{+4.0}_{-1.2} $  &  $ 0.239 \pm 0.021 $  &  $ 0.905 \pm 0.078 $  &  $ 65.11699 \pm 0.00047 $  &  $ 781.4039^{+0.0055}_{-0.0057} $  & 13 &  $ 71.0^{+41.0}_{-19.0} $  &  $ 0.284^{+0.059}_{-0.031} $  \\
269333648 &  $ 1.748 \pm 0.088 $  &  $ 0.209^{+0.055}_{-0.044} $  &  $ 1538.5239 \pm 0.0024 $  &  $ 2249.0554 \pm 0.0026 $  &  $ 11.72 \pm 0.67 $  &  $ 0.382 \pm 0.011 $  &  $ 0.64^{+0.1}_{-0.25} $  &  $ 64.59377 \pm 0.00032 $  &  $ 710.5315^{+0.0036}_{-0.0035} $  & 12 &  $ 65.0^{+24.0}_{-5.0} $  &  $ 0.26^{+0.1}_{-0.02} $  \\
323295479 &  $ 1.061 \pm 0.056 $  &  $ 0.78 \pm 0.18 $  &  $ 1622.92551 \pm 0.0009 $  &  $ 2365.43966 \pm 0.00093 $  &  $ 11.28 \pm 0.6 $  &  $ 0.2746 \pm 0.0037 $  &  $ 0.85 \pm 0.013 $  &  $ 67.50129 \pm 0.00012 $  &  $ 742.5142 \pm 0.0013 $  & 12 &  $ 83.0^{+41.0}_{-15.0} $  &  $ 0.204 \pm 0.058 $  \\
396720998 &  $ 0.16 \pm 0.1 $  &  $ 3.1^{+4.9}_{-2.2} $  &  $ 1399.2202 \pm 0.003 $  &  $ 2176.272 \pm 0.0031 $  &  $ 1.4 \pm 0.9 $  &  $ 0.189^{+0.018}_{-0.014} $  &  $ 0.46 \pm 0.32 $  &  $ 70.64107 \pm 0.00039 $  &  $ 777.0517 \pm 0.0043 $  & 12 &  $ 78.0^{+19.0}_{-13.0} $  &  $ 0.317^{+0.038}_{-0.018} $  \\
235058563 &  $ 1.468 \pm 0.067 $  &  $ 0.43 \pm 0.1 $  &  $ 1416.6106^{+0.0043}_{-0.0047} $  &  $ 2216.4423 \pm 0.0048 $  &  $ 11.47 \pm 0.61 $  &  $ 0.414 \pm 0.01 $  &  $ 0.38 \pm 0.23 $  &  $ 88.87019 \pm 0.00073 $  &  $ 799.8317 \pm 0.0066 $  & 10 &  $ 89.0^{+25.0}_{-9.0} $  &  $ 0.186^{+0.077}_{-0.022} $  \\
294097549 &  $ 1.147 \pm 0.053 $  &  $ 0.75^{+0.17}_{-0.14} $  &  $ 1657.7403^{+0.0052}_{-0.0056} $  &  $ 2256.3443^{+0.0037}_{-0.0035} $  &  $ 4.92 \pm 0.32 $  &  $ 0.3363^{+0.0099}_{-0.0087} $  &  $ 0.57^{+0.17}_{-0.33} $  &  $ 299.302 \pm 0.0033 $  &  $ 598.604^{+0.0068}_{-0.0064} $  & 3 &  $ 200.0^{+100.0}_{-0.0} $  &  $ 0.34^{+0.12}_{-0.0} $  \\
349091983 &  $ 1.498 \pm 0.072 $  &  $ 0.37^{+0.091}_{-0.076} $  &  $ 1603.1037 \pm 0.0044 $  &  $ 2152.1689^{+0.0044}_{-0.0047} $  &  $ 21.3^{+8.8}_{-4.8} $  &  $ 0.377^{+0.015}_{-0.014} $  &  $ 0.975^{+0.075}_{-0.058} $  &  $ 549.0649^{+0.0068}_{-0.0062} $  &  $ 549.0649^{+0.0068}_{-0.0062} $  & 1 &  ---  &  ---  \\
\bottomrule
\end{longtable}
\end{landscape}

==> 3.Results/table_2.tex <==

\begin{landscape}
\begin{longtable}{cccccccccccc}
\caption{Duotransit candidates.}\\
\toprule
ID & TIC ID & T\textsubscript{c1} & T\textsubscript{c2} & $\Delta$T\textsubscript{c} & Depth & Duration & \rpl\ & \gaia\ & \gaia\ RV  & Total SNR \\
 &  & (TBJD, [Sector])  & (TBJD, [Sector]) & (days) & (ppt) & (hours)  & (\rjup) & NSS & amp (\kms) & & \endhead
\hline

1 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=1504460}{1504460} & 1528.39739 [08] & 2261.11990 [35] & 732.72251 & 3.367 [08], 3.415 [35] & 3.78 & 0.83 & 0 & 13.84 & 14.82 \\
2 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=2669681}{2669681} & 1676.73302 [13] & 2044.45589 [27] & 367.72287 & 7.879 [13], 7.037 [27] & 9.69 & 1.61 & 0 & 36.15 & 41.8 \\
3 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=9844069}{9844069} & 1431.16511 [04] & 2148.92146 [31] & 717.75635 & 13.452 [04], 12.224 [31] & 7.20 & 1.80 & 0 & -- & 46.12 \\
4 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=13072758}{13072758} & 1455.59404 [05] & 2193.21295 [32] & 737.61891 & 7.023 [05], 6.755 [32] & 9.25 & 1.12 & 0 & 20.36 & 35.92 \\
5 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=13713700}{13713700} & 1536.98226 [08] & 2245.82903 [34] & 708.84677 & 7.234 [08], 4.700 [34] & 3.26 & 0.87 & 0 & -- & 35.92\\
6 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=14445414}{14445414} & 1497.55590 [07] & 2210.97620 [33] & 713.42031 & 2.317 [07], 2.179 [33] & 2.86 & 3.10 & 0 & 4.78 & 19.73 \\
7 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=20904104}{20904104} & 1390.11189 [03] & 2105.36177 [29] & 715.24989 & 0.738 [03], 1.065 [29] & 4.61 & 0.26 & 0 & 2.90 & 12.08 \\
8 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=25194908}{25194908} & 1402.29491 [03] & 2077.28343 [28] & 674.98852 & 6.590 [03], 6.266 [28] & 9.16 & 1.03 & 0 & -- & 11.84 \\
9 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=32179255}{32179255} & 1345.87922 [01] & 2068.45418 [28] & 722.57496 & 3.619 [01], 4.682 [28] & 3.71 & 4.52 & 2 & 49.01 & 31.43 \\
10 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=38138512}{38138512} & 1559.95080 [09] & 2300.02560 [36] & 740.07480 & 17.907 [09], 18.148 [36] & 6.73 & 1.67 & 0 & -- & 36.77 \\
11 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=39167176}{39167176} & 1470.62312 [06] & 2211.42630 [33] & 740.80317 & 7.282 [06], 8.112 [33] & 6.25 & 1.46 & 0 & 81.59 & 49.35\\
12 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=42428568}{42428568} & 1475.69109 [06] & 2224.32460 [33] & 748.63351 & 5.380 [06], 4.939 [33] & 10.20 & 2.16 & 0 & 16.42 & 40.79 \\
13 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=52195587}{52195587} & 1350.27811 [01] & 2107.61083 [29] & 757.33272 & 5.775 [01], 6.138 [29] & 9.07 & 0.84 & 0 & -- & 56.65 \\
14 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=66439839}{66439839} & 1386.34406 [03] & 2137.03203 [30] & 750.68798 & 6.227 [03], 5.420 [30] & 2.16 & 3.27 & 0 & 30.94 & 35.19 \\
15 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=67599025}{67599025} & 1404.02101 [03] & 2138.82557 [30] & 734.80456 & 6.684 [03], 7.345 [30] & 3.27 & 0.63 & 0 & 9.86 & 19.55 \\
16 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=70561926}{70561926} & 1523.06353 [08] & 2275.36040 [35] & 752.29687 & 16.290 [08], 16.053 [35] & 5.91 & 1.59 & 2 & 18.35 & 29.54 \\
17 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=71028120}{71028120} & 1445.81123 [05] & 2189.95412 [32] & 744.14289 & 1.238 [05], 1.025 [32] & 6.11 & 0.43 & 0 & 2.53 & 144.8 \\
18 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=77437543}{77437543} & 1456.70241 [05] & 2180.69226 [32] & 723.98986 & 9.825 [05], 9.326 [32] & 7.93 & 1.06 & 2 & 14.02 & 14.28 \\
19 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=81089255}{81089255} & 1509.94498 [07] & 2260.20690 [35] & 750.26191 & 7.318 [07], 6.372 [35] & 5.14 & 1.18 & 0 & 24.24 & 83.13 \\
20 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=100776118}{100776118} & 1472.81029 [06] & 2219.67770 [33] & 746.86740 & 13.264 [06], 13.070 [33] & 22.34 & 1.44 & 3 & 30.51 & 25.14 \\
21 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=101824521}{101824521} & 1620.35423 [11] & 2331.52820 [37] & 711.17397 & 9.396 [11], 9.103 [37] & 8.52 & 1.07 & 0 & -- & 177.47 \\
22 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=107113345}{107113345} & 1576.32832 [10] & 2317.29675 [37] & 740.96843 & 1.771 [10], 2.035 [37] & 1.77 & 0.54 & 0 & 19.10 & 34.34 \\
23 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=118339710}{118339710} & 1525.64667 [08] & 2249.54641 [34] & 723.89974 & 4.329 [08], 3.977 [34] & 8.68 & 1.00 & 0 & 4.13 & 12.5 \\
24 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=123763494}{123763494} & 1486.92891 [06] & 2209.76758 [33] & 722.83868 & 10.645 [06], 11.728 [33] & 2.47 & 5.15 & 0 & 15.94 & 62.67 \\
25 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=124029677}{124029677} & 1486.12090 [06] & 2218.00409 [33] & 731.88319 & 6.368 [06], 6.105 [33] & 4.58 & 1.01 & 0 & 11.35 & 37.36 \\
26 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=140215502}{140215502} & 1460.54584 [05] & 2194.44033 [32] & 733.89449 & 2.959 [05], 4.468 [32] & 7.14 & 0.51 & 0 & 9.83 & 46.16 \\
27 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=140750416}{140750416} & 1504.80151 [07] & 2245.39501 [34] & 740.59350 & 8.912 [07], 9.197 [34] & 3.85 & 0.77 & 0 & 11.19 & 32.98 \\
28 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=142278054}{142278054} & 1595.02504 [10] & 2310.35369 [37] & 715.32865 & 2.177 [10], 2.022 [37] & 4.82 & 1.01 & 0 & 7.72 & 30.13 \\
29 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=145006304}{145006304} & 1579.50384 [10] & 2318.24443 [37] & 738.74059 & 2.048 [10], 2.772 [37] & 5.19 & 0.48 & 0 & 6.03 & 23.25 \\
30 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=145913596}{145913596} & 1539.51696 [08] & 2242.69675 [34] & 703.17978 & 1.728 [08], 2.163 [34] & 8.50 & 0.71 & 0 & 5.83 & 25.32 \\
31 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=153838604}{153838604} & 1447.10227 [05] & 2176.13853 [32] & 729.03626 & 15.209 [05], 16.237 [32] & 2.61 & 3.36 & 0 & -- & 42.87 \\
32 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=156716001}{156716001} & 1485.40631 [06] & 2224.51833 [33] & 739.11201 & 2.652 [06], 3.037 [33] & 9.11 & 0.52 & 0 & 4.73 & 33.42 \\
33 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=157119927}{157119927} & 1591.62175 [10] & 2291.00613 [36] & 699.38439 & 5.445 [10], 6.897 [36] & 2.57 & 1.91 & 2 & 64.82 & 25.01 \\
34 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=157698565}{157698565} & 1494.57973 [07] & 2234.11360 [34] & 739.53387 & 9.825 [07], 9.338 [34] & 6.38 & 1.05 & 0 & 3.49 & 105.68 \\
35 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=159490807}{159490807} & 1606.22551 [11] & 2355.93796 [38] & 749.71245 & 5.155 [11], 5.184 [38] & 5.38 & 1.40 & 0 & 6.08 & 45.05 \\
36 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=161169240}{161169240} & 1328.25945 [01] & 2083.31754 [28] & 755.05809 & 9.707 [01], 10.134 [28] & 7.82 & 1.14 & 0 & 32.37 & 52.27 \\
37 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=176518126}{176518126} & 1489.05533 [06] & 2219.53761 [33] & 730.48228 & 3.565 [06], 3.244 [33] & 5.61 & 0.75 & 0 & 9.38 & 32.89 \\
38 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=188620407}{188620407} & 1375.48660 [02] & 2461.70715 [42] & 1086.22055 & 5.467 [02], 4.512 [42] & 6.08 & 0.89 & 0 & 11.56 & 50.40 \\
39 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=193318850}{193318850} & 1553.77031 [09] & 2292.51011 [36] & 738.73979 & 6.916 [09], 7.143 [36] & 3.89 & 0.62 & 0 & -- & 17.05 \\
40 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=199738560}{199738560} & 1390.85958 [03] & 2121.95440 [30] & 731.09482 & 13.593 [03], 13.638 [30] & 9.89 & 2.24 & 0 & -- & 36.92 \\
41 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=207783865}{207783865} & 1608.93692 [11] & 2354.11345 [38] & 745.17652 & 17.211 [11], 17.729 [38] & 1.99 & 1.37 & 2 & 13.91 & 95.83 \\
42 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=211376134}{211376134} & 1341.31067 [01] & 2078.16253 [28] & 736.85186 & 21.890 [01], 21.767 [28] & 3.40 & 4.39 & 0 & 68.51 & 210.93 \\
43 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=211409161}{211409161} & 1335.10057 [01] & 2070.36583 [28] & 735.26527 & 13.629 [01], 12.232 [28] & 2.14 & 1.00 & 0 & 38.64 & 38.49 \\
44 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=215402824}{215402824} & 1413.62655 [04] & 2169.04205 [31] & 755.41550 & 5.589 [04], 9.955 [31] & 1.87 & 3.91 & 0 & -- & 12.73 \\
45 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=218977148}{218977148} & 1355.47069 [02] & 2090.09772 [29] & 734.62703 & 5.597 [02], 4.944 [29] & 8.13 & 1.12 & 0 & -- & 22.83 \\
46 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=220622886}{220622886} & 1479.52544 [06] & 2204.58502 [33] & 725.05958 & 4.324 [06], 3.501 [33] & 4.43 & 9.83 & 0 & 65.91 & 18.89 \\
47 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=221915858}{221915858} & 1643.35799 [12] & 2372.55118 [39] & 729.19319 & 5.737 [12], 5.526 [39] & 3.05 & 1.88 & 0 & 60.96 & 33.79 \\
48 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=224279805}{224279805} & 1369.72941 [02] & 2105.21571 [29] & 735.48631 & 6.392 [02], 6.618 [29] & 5.93 & 0.94 & 0 & 17.77 & 30.43 \\
49 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=235058563}{235058563} & 1416.61066 [04] & 2216.44259 [33] & 799.83193 & 6.164 [04], 5.630 [33] & 10.17 & 1.06 & 0 & -- & 27.17 \\
50 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=237605045}{237605045} & 1489.04268 [06] & 2210.29724 [33] & 721.25457 & 6.212 [06], 7.014 [33] & 4.42 & 10.34 & 0 & 36.88 & 68.84 \\
51 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=242241304}{242241304} & 1623.07095 [11] & 2345.37403 [38] & 722.30308 & 6.158 [11], 6.186 [38] & 4.72 & 0.89 & 0 & 7.03 & 28.72 \\
52 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=251057075}{251057075} & 1426.31846 [04] & 2154.02335 [31] & 727.70489 & 1.986 [04], 2.348 [31] & 4.42 & 0.36 & 0 & 7.82 & 15.54 \\
53 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=256912435}{256912435} & 1623.43775 [11] & 2338.70979 [38] & 715.27204 & 20.396 [11], 21.562 [38] & 2.72 & 4.90 & 0 & 46.85 & 57.70 \\
54 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=265465927}{265465927} & 1342.64749 [01] & 2058.60913 [27] & 715.96164 & 8.678 [01], 8.720 [27] & 6.05 & 1.06 & 0 & 19.67 & 38.93 \\
55 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=265466589}{265466589} & 1352.52439 [01] & 2037.86660 [27] & 685.34222 & 6.818 [01], 6.664 [27] & 4.14 & 0.75 & 0 & -- & 13.71 \\
56 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=268534931}{268534931} & 1398.29475 [03] & 2139.09941 [30] & 740.80465 & 5.829 [03], 6.133 [30] & 7.82 & 0.58 & 0 & 25.23 & 29.74 \\
57 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=269333648}{269333648} & 1538.52419 [08] & 2249.05416 [34] & 710.52997 & 4.162 [08], 4.032 [34] & 9.46 & 1.07 & 0 & 3.20 & 54.46 \\
58 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=275878706}{275878706} & 1621.08010 [11] & 2341.78257 [38] & 720.70247 & 6.544 [11], 5.320 [38] & 4.38 & 4.15 & 1 & 21.81 & 20.68 \\
59 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=279727635}{279727635} & 1343.22676 [01] & 2124.62930 [30] & 781.40254 & 7.181 [01], 6.789 [30] & 5.71 & 2.34 & 0 & -- & 28.36 \\
60 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=287204963}{287204963} & 1402.93640 [03] & 2132.33438 [30] & 729.39798 & 11.498 [03], 10.182 [30] & 4.73 & 1.05 & 0 & -- & 17.86 \\
61 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=289840544}{289840544} & 1331.28977 [01] & 2083.28790 [28] & 751.99813 & 2.702 [01], 1.997 [28] & 2.99 & 2.95 & 0 & 6.43 & 17.85 \\
62 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=290165539}{290165539} & 1332.75615 [01] & 2067.97094 [28] & 735.21479 & 13.627 [01], 15.056 [28] & 11.50 & 2.23 & 0 & 45.38 & 92.47 \\
63 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=292719109}{292719109} & 1499.70159 [07] & 2222.31933 [33] & 722.61775 & 2.859 [07], 2.677 [33] & 9.08 & 1.02 & 0 & 2.50 & 45.22 \\
64 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=294097549}{294097549} & 1657.74149 [13] & 2256.34250 [35] & 598.60101 & 1.977 [13], 1.426 [35] & 7.96 & 0.45 & 0 & 4.14 & 22.63 \\
65 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=296737508}{296737508} & 1538.00622 [08] & 2271.99796 [35] & 733.99174 & 2.021 [08], 1.854 [35] & 5.65 & 0.50 & 0 & 1.12 & 41.08 \\
66 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=300394149}{300394149} & 1576.88642 [10] & 2325.42588 [37] & 748.53947 & 2.051 [10], 2.195 [37] & 13.40 & 0.61 & 0 & 4.92 & 36.29 \\
67 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=303317324}{303317324} & 1365.17582 [02] & 2104.34337 [29] & 739.16755 & 1.360 [02], 1.323 [29] & 5.74 & 0.28 & 0 & 1.16 & 22.71 \\
68 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=304339227}{304339227} & 1673.33918 [13] & 2388.01911 [39] & 714.67993 & 0.522 [13], 0.464 [39] & 5.79 & 0.28 & 0 & 2.19 & 13.81 \\
69 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=306249066}{306249066} & 1593.97611 [10] & 2326.51397 [37] & 732.53786 & 7.873 [10], 7.061 [37] & 4.03 & 1.00 & 0 & 7.34 & 49.32 \\
70 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=313671132}{313671132} & 1604.35452 [11] & 2337.72693 [38] & 733.37241 & 3.408 [11], 3.506 [38] & 5.70 & 0.74 & 0 & 7.02 & 27.41 \\
71 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=317923092}{317923092} & 1479.81772 [06] & 2209.42617 [33] & 729.60845 & 4.358 [06], 6.715 [33] & 12.96 & 6.31 & 0 & 35.10 & 30.15 \\
72 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=323295479}{323295479} & 1622.92483 [11] & 2365.44036 [39] & 742.51554 & 8.727 [11], 8.609 [39] & 6.51 & 1.01 & 0 & 2.43 & 138.65 \\
73 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=332697924}{332697924} & 1445.74977 [05] & 2178.22194 [32] & 732.47218 & 1.042 [05], 1.423 [32] & 6.63 & 0.44 & 0 & 5.60 & 11.96 \\
74 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=333736132}{333736132} & 1551.55292 [09] & 2283.54681 [36] & 731.99390 & 15.856 [09], 16.440 [36] & 2.96 & 0.95 & 0 & 13.92 & 55.96 \\
75 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=339399841}{339399841} & 1662.10984 [13] & 2043.59486 [27] & 381.48503 & 4.773 [13], 6.471 [27] & 6.66 & 1.13 & 0 & -- & 21.13 \\
76 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=349091983}{349091983} & 1603.10253 [11] & 2152.16754 [31] & 549.06501 & 8.301 [11], 8.133 [31] & 9.52 & 4.91 & 0 & -- & 44.11 \\
77 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=366322247}{366322247} & 1618.29549 [11] & 2352.41070 [38] & 734.11521 & 4.569 [11], 4.223 [38] & 2.87 & 12.83 & 0 & -- & 45.35 \\
78 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=381553868}{381553868} & 1677.32594 [13] & 2367.57869 [39] & 690.25274 & 5.653 [13], 6.030 [39] & 6.49 & 1.12 & 0 & 9.94 & 22.00 \\
79 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=393229954}{393229954} & 1446.79953 [05] & 2204.55168 [33] & 757.75214 & 8.172 [05], 6.652 [33] & 2.67 & 0.79 & 0 & 12.97 & 33.63 \\
80 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=394340183}{394340183} & 1664.84261 [13] & 2389.11243 [39] & 724.26982 & 11.255 [13], 10.820 [39] & 8.65 & 1.04 & 0 & 6.77 & 85.43 \\
81 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=396720998}{396720998} & 1399.21966 [03] & 2176.27178 [32] & 777.05212 & 6.360 [03], 6.082 [32] & 4.33 & 0.13 & 0 & -- & 6.44 \\
82 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=404518509}{404518509} & 1431.26615 [04] & 2134.88294 [30] & 703.61679 & 0.842 [04], 0.598 [30] & 5.02 & 0.24 & 0 & 0.93 & 22.52 \\
83 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=412386707}{412386707} & 1493.95365 [07] & 2240.57066 [34] & 746.61701 & 3.442 [07], 3.587 [34] & 5.23 & 1.08 & 0 & 6.18 & 28.97\\
84 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=437293313}{437293313} & 1578.44737 [10] & 2328.08914 [37] & 749.64177 & 9.891 [10], 8.462 [37] & 6.58 & 0.81 & 0 & -- & 26.34 \\
85 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=439491923}{439491923} & 1405.41115 [03] & 2116.79038 [30] & 711.37923 & 11.608 [03], 11.766 [30] & 6.70 & 1.33 & 0 & -- & 36.20 \\
86 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=442893494}{442893494} & 1472.65885 [06] & 2194.38454 [32] & 721.72570 & 5.776 [06], 6.458 [32] & 7.70 & 1.01 & 0 & -- & 24.76 \\
87 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=457649900}{457649900} & 1606.96984 [11] & 2355.79522 [38] & 748.82538 & 2.857 [11], 2.945 [38] & 7.61 & 4.54 & 0 & 13.11 & 29.26 \\
88 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=466206508}{466206508} & 1679.34576 [13] & 2054.97133 [27] & 375.62557 & 11.214 [13], 9.274 [27] & 8.03 & 1.24 & 0 & 12.81 & 64.68 \\
\bottomrule
\label{tab:candidate_events}
\end{longtable}
\end{landscape}

==> referee.tex <==
We would like to thank the referee for reviewing the manuscript and their suggested improvements.  We have implemented all the suggested corrections and changes. We have produced a new PDF manuscript with all amendments in yellow highlighted font.  We also list all the changes in detail below:


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% - Given that the pre-vetting step is the most significant in terms of reduction of the number of candidates (it reduces the number of candidates by more than an order of magnitude) and that this step is purely done by visual inspection, it would be useful if the authors report and comment a few examples of false positive detections identified during this step.

% We have added Figure 2 to the paper and descriptive text, which includes examples of an asteroid, stellar variability and systematic detection by the algorithm, all of which were identified during the pre-vetting step.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% - I think figure 5 should more appropriately present the color magnitude diagram corrected for reddening and extinction rather than just the observed color magnitude diagram.

% We have updated figure 5 and its caption accordingly, using corrected values of extinction and reddening from Gaia DR3 derivations from gspphot. Where values for these were not available for candidates, we revert to the calculation from parallax values and note this in the table caption (and refer the reader to Table A1 where the available distance values from DR3 can be seen).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% - I think that in Section 5 it would be useful to report and discuss also the distribution of distances of the candidates and of the TESS confirmed exoplanets which can be obtained from Gaia DR3.

% We have added the values of distance from the Gaia DR3 catalog to table A1, created a histogram (Figure 11) and added description to the text in section 5.1.

==> tables.tex <==

\clearpage
\onecolumn



\begin{longtable}{ccccccccc}
\caption{Duotransit candidates stellar properties.}\\
\toprule
ID & TIC ID & TOI/CTOI & RA (deg) & Dec (deg) & \tmag\ & \rstar\ (\rsun) & \teff\ (K) & N\textsubscript{sec} \endhead
\hline

1 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=1504460}{1504460} & -- & 131.96578 & -23.98953  & 11.63 & 1.50 & 6218 & 2 \\
2 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=2669681}{2669681} & -- & 289.36801 & -28.58032  & 11.47 & 1.88 & 5160 & 2 \\
3 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=9844069}{9844069} & -- & 48.03923 & -11.68080  & 12.96 & 1.61 & 5665 & 2 \\
4 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=13072758}{13072758} & CTOI & 76.08837 & -29.03421  & 12.22 & 1.43 & 6313 & 2 \\
5 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=13713700}{13713700} & -- & 133.63960 & -7.94134  & 12.29 & 0.97 & 5864 & 2 \\
6 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=14445414}{14445414} & -- & 110.82089 & 12.66321  & 11.02 & 1.31 & 6425 & 2 \\
7 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=20904104}{20904104} & -- & 7.41368 & -19.36625  & 9.76 & 0.88 & 5628 & 2 \\
8 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=25194908}{25194908} & -- & 63.90318 & -66.35192  & 12.46 & 1.32 & 6309 & 24 \\
9 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=32179255}{32179255} & -- & 332.03964 & -29.60930  & 10.52 & 1.75 & 5989 & 2 \\
10 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=38138512}{38138512} & -- & 170.41830 & -4.19721  & 12.94 & 1.34 & 6300 & 2 \\
11 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=39167176}{39167176} & -- & 88.32738 & -3.79767  & 12.01 & 1.56 & 8416 & 2 \\
12 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=42428568}{42428568} & -- & 96.29347 & -3.76657  & 10.83 & 2.16 & 6686 & 2 \\
13 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=52195587}{52195587} & -- & 19.24834 & -66.16364  & 12.25 & 1.20 & 5736 & 4 \\
14 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=66439839}{66439839} & -- & 14.47851 & -30.32314  & 11.97 & 1.03 & 5882 & 3 \\
15 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=67599025}{67599025} & CTOI & 17.69268 & -31.50549  & 11.96 & 0.78 & 4816 & 2 \\
16 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=70561926}{70561926} & -- & 139.25588 & -26.70065  & 11.00 & 1.35 & 6386 & 2 \\
17 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=71028120}{71028120} & -- & 66.12741 & -11.98354  & 10.44 & 1.37 & 5596 & 2 \\
18 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=77437543}{77437543} & TOI-2490 & 73.12441 & -36.25715  & 11.28 & 1.17 & 5459 & 3 \\
19 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=81089255}{81089255} & CTOI & 122.69418 & -43.85349  & 11.84 & 1.43 & 7459 & 4 \\
20 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=100776118}{100776118} & CTOI & 88.31784 & -34.51847  & 11.51 & 1.25 & 6439 & 4 \\
21 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=101824521}{101824521} & -- & 206.00402 & -26.49780  & 12.61 & 1.23 & 5553 & 2 \\
22 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=107113345}{107113345} & -- & 183.03410 & -32.66283  & 10.34 & 1.31 & 6696 & 2 \\
23 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=118339710}{118339710} & CTOI & 129.57204 & -23.55023  & 10.35 & 1.56 & 6119 & 3 \\
24 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=123763494}{123763494} & -- & 90.30269 & -21.23587  & 11.73 & 1.22 & 5568 & 2 \\
25 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=124029677}{124029677} & TOI-5153 & 91.54028 & -19.95330  & 11.21 & 1.38 & 6408 & 2 \\
26 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=140215502}{140215502} & CTOI & 85.15071 & -34.76638  & 11.23 & 0.93 & 5528 & 4 \\
27 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=140750416}{140750416} & -- & 116.43818 & -23.14302  & 11.81 & 0.87 & 5331 & 2 \\
28 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=142278054}{142278054} & -- & 180.76256 & -33.34303  & 10.28 & 2.39 & 6400 & 2 \\
29 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=145006304}{145006304} & -- & 193.33448 & -39.73471  & 11.30 & 1.12 & 6340 & 2 \\
30 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=145913596}{145913596} & -- & 123.12977 & -30.55547  & 10.17 & 1.45 & 6467 & 4 \\
31 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=153838604}{153838604} & -- & 68.07396 & -47.60877  & 12.48 & 0.91 & 5649 & 4 \\
32 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=156716001}{156716001} & -- & 103.10631 & -39.68757  & 10.90 & 1.08 & 6129 & 4 \\
33 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=157119927}{157119927} & -- & 175.21548 & -31.13741  & 11.64 & 1.04 & 5765 & 2 \\
34 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=157698565}{157698565} & TOI-2589 & 107.48825 & -37.23098  & 10.72 & 1.07 & 5938 & 3 \\
35 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=159490807}{159490807} & -- & 220.23493 & -39.37566  & 10.57 & 1.69 & 6556 & 2 \\
36 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=161169240}{161169240} & CTOI & 339.35732 & -53.31878  & 12.12 & 1.19 & 5952 & 2 \\
37 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=176518126}{176518126} & -- & 87.18320 & -0.49503  & 10.48 & 1.36 & 7927 & 2 \\
38 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=188620407}{188620407} & CTOI & 350.05108 & -13.04939  & 11.57 & 1.31 & 6169 & 3 \\
39 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=193318850}{193318850} & -- & 177.73016 & -16.74172  & 12.76 & 0.79 & 5560 & 2 \\
40 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=199738560}{199738560} & -- & 23.05401 & -44.07057  & 13.09 & 1.90 & 5443 & 3 \\
41 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=207783865}{207783865} & -- & 207.06088 & -54.42060  & 10.54 & 1.04 & 5936 & 2 \\
42 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=211376134}{211376134} & -- & 320.74107 & -32.48809  & 10.17 & 1.12 & 6286 & 2 \\
43 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=211409161}{211409161} & -- & 321.77681 & -30.52732  & 10.44 & 0.78 & 4660 & 2 \\
44 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=215402824}{215402824} & -- & 43.06240 & -36.28874  & 12.97 & 1.33 & 6180 & 4 \\
45 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=218977148}{218977148} & -- & 349.53308 & -33.13686  & 12.58 & 1.61 & 6214 & 2 \\
46 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=220622886}{220622886} & -- & 84.89306 & -42.68114  & 12.00 & 2.56 & 5671 & 3 \\
47 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=221915858}{221915858} & -- & 249.51302 & -54.35785  & 10.07 & 2.47 & 9475 & 2 \\
48 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=224279805}{224279805} & CTOI & 355.73864 & -40.77217  & 12.15 & 1.20 & 5591 & 2 \\
49 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=235058563}{235058563} & -- & 83.51699 & -50.12157  & 12.43 & 1.47 & 6438 & 6 \\
50 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=237605045}{237605045} & -- & 103.28961 & 2.05465  & 10.29 & 2.92 & 6577 & 2 \\
51 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=242241304}{242241304} & CTOI & 211.58509 & -43.04474  & 11.81 & 1.14 & 5781 & 2 \\
52 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=251057075}{251057075} & -- & 36.17507 & -5.85401  & 11.05 & 0.84 & 5225 & 2 \\
53 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=256912435}{256912435} & -- & 200.54621 & -55.21835  & 11.80 & 1.19 & 5650 & 2 \\
54 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=265465927}{265465927} & CTOI & 320.91656 & -62.92377  & 12.08 & 1.16 & 6099 & 2 \\
55 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=265466589}{265466589} & -- & 321.07935 & -64.47431  & 12.61 & 1.03 & 5834 & 2 \\
56 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=268534931}{268534931} & CTOI & 15.12618 & -23.17953  & 12.22 & 0.78 & 5179 & 2 \\
57 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=269333648}{269333648} & TOI-2529 & 118.99443 & -52.35491  & 10.67 & 1.75 & 5822 & 6 \\
58 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=275878706}{275878706} & -- & 207.90184 & -44.31443  & 12.17 & 0.93 & 5038 & 2 \\
59 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=279727635}{279727635} & -- & 50.59176 & -64.44435  & 12.50 & 1.05 & 5851 & 6 \\
60 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=287204963}{287204963} & -- & 30.28722 & -11.88352  & 13.25 & 1.04 & 5344 & 2 \\
61 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=289840544}{289840544} & -- & 317.54548 & -26.39994  & 10.64 & 1.75 & 5989 & 2 \\
62 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=290165539}{290165539} & -- & 319.85211 & -25.59712  & 11.99 & 1.33 & 5895 & 2 \\
63 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=292719109}{292719109} & -- & 107.41596 & 3.56756  & 10.10 & 2.08 & 6216 & 2 \\
64 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=294097549}{294097549} & -- & 107.67004 & -55.79671  & 10.47 & 1.15 & 5872 & 13 \\
65 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=296737508}{296737508} & CTOI & 142.17926 & -14.68643  & 9.20 & 1.27 & 5700 & 2 \\
66 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=300394149}{300394149} & -- & 170.74699 & -52.69860  & 10.13 & 1.42 & 5997 & 2 \\
67 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=303317324}{303317324} & TOI-4310 & 351.90369 & -25.50809  & 9.50 & 0.72 & 4159 & 2 \\
68 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=304339227}{304339227} & TOI-4629 & 275.94385 & -68.34489  & 8.66 & 1.13 & 6012 & 2 \\
69 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=306249066}{306249066} & -- & 166.72853 & -54.73883  & 10.54 & 1.14 & 6139 & 2 \\
70 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=313671132}{313671132} & -- & 202.15822 & -62.16990  & 10.08 & 1.22 & 5878 & 2 \\
71 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=317923092}{317923092} & -- & 89.85183 & -14.90606  & 12.26 & 1.34 & 7604 & 2 \\
72 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=323295479}{323295479} & TOI-1861 & 130.79865 & -83.06100  & 9.95 & 1.06 & 5684 & 5 \\
73 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=332697924}{332697924} & -- & 63.26121 & -12.45925  & 11.00 & 1.32 & 6266 & 2 \\
74 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=333736132}{333736132} & CTOI & 170.27654 & -26.06656  & 12.07 & 0.76 & 4722 & 2 \\
75 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=339399841}{339399841} & -- & 296.07049 & -62.81358  & 12.35 & 1.55 & 5686 & 2 \\
76 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=349091983}{349091983} & -- & 107.70509 & -61.35237  & 12.29 & 1.50 & 6083 & 24 \\
77 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=366322247}{366322247} & -- & 219.18211 & -31.53615  & 10.09 & 2.92 & 6293 & 2 \\
78 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=381553868}{381553868} & -- & 269.77432 & -50.92122  & 11.85 & 1.59 & 6355 & 2 \\
79 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=393229954}{393229954} & -- & 86.74486 & -46.71186  & 11.77 & 0.90 & 5571 & 5 \\
80 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=394340183}{394340183} & -- & 39.32208 & -79.45825  & 10.95 & 1.04 & 6325 & 2 \\
81 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=396720998}{396720998} & TOI-709 & 65.65532 & -54.14718  & 13.99 & 0.15 & 50000 & 6 \\
82 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=404518509}{404518509} & TOI-4320 & 51.64036 & -43.61357  & 8.60 & 1.04 & 5871 & 4 \\
83 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=412386707}{412386707} & -- & 110.48705 & -23.41404  & 10.92 & 1.96 & 6304 & 2 \\
84 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=437293313}{437293313} & -- & 191.22344 & -22.61769  & 12.97 & 0.94 & 5536 & 2 \\
85 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=439491923}{439491923} & -- & 21.38365 & -18.14711  & 12.87 & 1.26 & 5944 & 2 \\
86 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=442893494}{442893494} & -- & 80.00938 & -16.21927  & 12.41 & 1.39 & 6322 & 3 \\
87 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=457649900}{457649900} & TOI-4958 & 217.99906 & -51.07439  & 10.75 & 2.11 & 6713 & 2 \\
88 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=466206508}{466206508} & TOI-5542 & 302.79848 & -61.13545  & 11.85 & 1.27 & 5393 & 2 \\
\bottomrule
%\label{tab:candidate_stellar}
\end{longtable}




\begin{landscape}
\begin{longtable}{cccccccccccc}
\caption{Duotransit candidates.}\\
\toprule
ID & TIC ID & T\textsubscript{c1} & T\textsubscript{c2} & $\Delta$T\textsubscript{c} & Depth & Duration & \rpl\ & \gaia\ & \gaia\ RV  \\
 &  & (TBJD, [Sector])  & (TBJD, [Sector]) & (days) & (ppt) & (hours)  & (\rjup) & non-single star & amplitude (\kms) & \endhead
\hline

1 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=1504460}{1504460} & 1528.39739 [08] & 2261.11990 [35] & 732.72251 & 3.367 [08], 3.415 [35] & 3.78 & 0.83 & 0 & 13.84 \\
2 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=2669681}{2669681} & 1676.73302 [13] & 2044.45589 [27] & 367.72287 & 7.879 [13], 7.037 [27] & 9.69 & 1.61 & 0 & 36.15 \\
3 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=9844069}{9844069} & 1431.16511 [04] & 2148.92146 [31] & 717.75635 & 13.452 [04], 12.224 [31] & 7.20 & 1.80 & 0 & -- \\
4 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=13072758}{13072758} & 1455.59404 [05] & 2193.21295 [32] & 737.61891 & 7.023 [05], 6.755 [32] & 9.25 & 1.12 & 0 & 20.36 \\
5 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=13713700}{13713700} & 1536.98226 [08] & 2245.82903 [34] & 708.84677 & 7.234 [08], 4.700 [34] & 3.26 & 0.87 & 0 & -- \\
6 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=14445414}{14445414} & 1497.55590 [07] & 2210.97620 [33] & 713.42031 & 2.317 [07], 2.179 [33] & 2.86 & 3.10 & 0 & 4.78 \\
7 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=20904104}{20904104} & 1390.11189 [03] & 2105.36177 [29] & 715.24989 & 0.738 [03], 1.065 [29] & 4.61 & 0.26 & 0 & 2.90 \\
8 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=25194908}{25194908} & 1402.29491 [03] & 2077.28343 [28] & 674.98852 & 6.590 [03], 6.266 [28] & 9.16 & 1.03 & 0 & -- \\
9 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=32179255}{32179255} & 1345.87922 [01] & 2068.45418 [28] & 722.57496 & 3.619 [01], 4.682 [28] & 3.71 & 4.52 & 2 & 49.01 \\
10 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=38138512}{38138512} & 1559.95080 [09] & 2300.02560 [36] & 740.07480 & 17.907 [09], 18.148 [36] & 6.73 & 1.67 & 0 & -- \\
11 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=39167176}{39167176} & 1470.62312 [06] & 2211.42630 [33] & 740.80317 & 7.282 [06], 8.112 [33] & 6.25 & 1.46 & 0 & 81.59 \\
12 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=42428568}{42428568} & 1475.69109 [06] & 2224.32460 [33] & 748.63351 & 5.380 [06], 4.939 [33] & 10.20 & 2.16 & 0 & 16.42 \\
13 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=52195587}{52195587} & 1350.27811 [01] & 2107.61083 [29] & 757.33272 & 5.775 [01], 6.138 [29] & 9.07 & 0.84 & 0 & -- \\
14 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=66439839}{66439839} & 1386.34406 [03] & 2137.03203 [30] & 750.68798 & 6.227 [03], 5.420 [30] & 2.16 & 3.27 & 0 & 30.94 \\
15 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=67599025}{67599025} & 1404.02101 [03] & 2138.82557 [30] & 734.80456 & 6.684 [03], 7.345 [30] & 3.27 & 0.63 & 0 & 9.86 \\
16 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=70561926}{70561926} & 1523.06353 [08] & 2275.36040 [35] & 752.29687 & 16.290 [08], 16.053 [35] & 5.91 & 1.59 & 2 & 18.35 \\
17 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=71028120}{71028120} & 1445.81123 [05] & 2189.95412 [32] & 744.14289 & 1.238 [05], 1.025 [32] & 6.11 & 0.43 & 0 & 2.53 \\
18 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=77437543}{77437543} & 1456.70241 [05] & 2180.69226 [32] & 723.98986 & 9.825 [05], 9.326 [32] & 7.93 & 1.06 & 2 & 14.02 \\
19 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=81089255}{81089255} & 1509.94498 [07] & 2260.20690 [35] & 750.26191 & 7.318 [07], 6.372 [35] & 5.14 & 1.18 & 0 & 24.24 \\
20 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=100776118}{100776118} & 1472.81029 [06] & 2219.67770 [33] & 746.86740 & 13.264 [06], 13.070 [33] & 22.34 & 1.44 & 3 & 30.51 \\
21 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=101824521}{101824521} & 1620.35423 [11] & 2331.52820 [37] & 711.17397 & 9.396 [11], 9.103 [37] & 8.52 & 1.07 & 0 & -- \\
22 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=107113345}{107113345} & 1576.32832 [10] & 2317.29675 [37] & 740.96843 & 1.771 [10], 2.035 [37] & 1.77 & 0.54 & 0 & 19.10 \\
23 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=118339710}{118339710} & 1525.64667 [08] & 2249.54641 [34] & 723.89974 & 4.329 [08], 3.977 [34] & 8.68 & 1.00 & 0 & 4.13 \\
24 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=123763494}{123763494} & 1486.92891 [06] & 2209.76758 [33] & 722.83868 & 10.645 [06], 11.728 [33] & 2.47 & 5.15 & 0 & 15.94 \\
25 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=124029677}{124029677} & 1486.12090 [06] & 2218.00409 [33] & 731.88319 & 6.368 [06], 6.105 [33] & 4.58 & 1.01 & 0 & 11.35 \\
26 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=140215502}{140215502} & 1460.54584 [05] & 2194.44033 [32] & 733.89449 & 2.959 [05], 4.468 [32] & 7.14 & 0.51 & 0 & 9.83 \\
27 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=140750416}{140750416} & 1504.80151 [07] & 2245.39501 [34] & 740.59350 & 8.912 [07], 9.197 [34] & 3.85 & 0.77 & 0 & 11.19 \\
28 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=142278054}{142278054} & 1595.02504 [10] & 2310.35369 [37] & 715.32865 & 2.177 [10], 2.022 [37] & 4.82 & 1.01 & 0 & 7.72 \\
29 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=145006304}{145006304} & 1579.50384 [10] & 2318.24443 [37] & 738.74059 & 2.048 [10], 2.772 [37] & 5.19 & 0.48 & 0 & 6.03 \\
30 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=145913596}{145913596} & 1539.51696 [08] & 2242.69675 [34] & 703.17978 & 1.728 [08], 2.163 [34] & 8.50 & 0.71 & 0 & 5.83 \\
31 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=153838604}{153838604} & 1447.10227 [05] & 2176.13853 [32] & 729.03626 & 15.209 [05], 16.237 [32] & 2.61 & 3.36 & 0 & -- \\
32 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=156716001}{156716001} & 1485.40631 [06] & 2224.51833 [33] & 739.11201 & 2.652 [06], 3.037 [33] & 9.11 & 0.52 & 0 & 4.73 \\
33 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=157119927}{157119927} & 1591.62175 [10] & 2291.00613 [36] & 699.38439 & 5.445 [10], 6.897 [36] & 2.57 & 1.91 & 2 & 64.82 \\
34 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=157698565}{157698565} & 1494.57973 [07] & 2234.11360 [34] & 739.53387 & 9.825 [07], 9.338 [34] & 6.38 & 1.05 & 0 & 3.49 \\
35 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=159490807}{159490807} & 1606.22551 [11] & 2355.93796 [38] & 749.71245 & 5.155 [11], 5.184 [38] & 5.38 & 1.40 & 0 & 6.08 \\
36 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=161169240}{161169240} & 1328.25945 [01] & 2083.31754 [28] & 755.05809 & 9.707 [01], 10.134 [28] & 7.82 & 1.14 & 0 & 32.37 \\
37 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=176518126}{176518126} & 1489.05533 [06] & 2219.53761 [33] & 730.48228 & 3.565 [06], 3.244 [33] & 5.61 & 0.75 & 0 & 9.38 \\
38 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=188620407}{188620407} & 1375.48660 [02] & 2461.70715 [42] & 1086.22055 & 5.467 [02], 4.512 [42] & 6.08 & 0.89 & 0 & 11.56 \\
39 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=193318850}{193318850} & 1553.77031 [09] & 2292.51011 [36] & 738.73979 & 6.916 [09], 7.143 [36] & 3.89 & 0.62 & 0 & -- \\
40 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=199738560}{199738560} & 1390.85958 [03] & 2121.95440 [30] & 731.09482 & 13.593 [03], 13.638 [30] & 9.89 & 2.24 & 0 & -- \\
41 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=207783865}{207783865} & 1608.93692 [11] & 2354.11345 [38] & 745.17652 & 17.211 [11], 17.729 [38] & 1.99 & 1.37 & 2 & 13.91 \\
42 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=211376134}{211376134} & 1341.31067 [01] & 2078.16253 [28] & 736.85186 & 21.890 [01], 21.767 [28] & 3.40 & 4.39 & 0 & 68.51 \\
43 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=211409161}{211409161} & 1335.10057 [01] & 2070.36583 [28] & 735.26527 & 13.629 [01], 12.232 [28] & 2.14 & 1.00 & 0 & 38.64 \\
44 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=215402824}{215402824} & 1413.62655 [04] & 2169.04205 [31] & 755.41550 & 5.589 [04], 9.955 [31] & 1.87 & 3.91 & 0 & -- \\
45 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=218977148}{218977148} & 1355.47069 [02] & 2090.09772 [29] & 734.62703 & 5.597 [02], 4.944 [29] & 8.13 & 1.12 & 0 & -- \\
46 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=220622886}{220622886} & 1479.52544 [06] & 2204.58502 [33] & 725.05958 & 4.324 [06], 3.501 [33] & 4.43 & 9.83 & 0 & 65.91 \\
47 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=221915858}{221915858} & 1643.35799 [12] & 2372.55118 [39] & 729.19319 & 5.737 [12], 5.526 [39] & 3.05 & 1.88 & 0 & 60.96 \\
48 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=224279805}{224279805} & 1369.72941 [02] & 2105.21571 [29] & 735.48631 & 6.392 [02], 6.618 [29] & 5.93 & 0.94 & 0 & 17.77 \\
49 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=235058563}{235058563} & 1416.61066 [04] & 2216.44259 [33] & 799.83193 & 6.164 [04], 5.630 [33] & 10.17 & 1.06 & 0 & -- \\
50 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=237605045}{237605045} & 1489.04268 [06] & 2210.29724 [33] & 721.25457 & 6.212 [06], 7.014 [33] & 4.42 & 10.34 & 0 & 36.88 \\
51 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=242241304}{242241304} & 1623.07095 [11] & 2345.37403 [38] & 722.30308 & 6.158 [11], 6.186 [38] & 4.72 & 0.89 & 0 & 7.03 \\
52 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=251057075}{251057075} & 1426.31846 [04] & 2154.02335 [31] & 727.70489 & 1.986 [04], 2.348 [31] & 4.42 & 0.36 & 0 & 7.82 \\
53 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=256912435}{256912435} & 1623.43775 [11] & 2338.70979 [38] & 715.27204 & 20.396 [11], 21.562 [38] & 2.72 & 4.90 & 0 & 46.85 \\
54 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=265465927}{265465927} & 1342.64749 [01] & 2058.60913 [27] & 715.96164 & 8.678 [01], 8.720 [27] & 6.05 & 1.06 & 0 & 19.67 \\
55 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=265466589}{265466589} & 1352.52439 [01] & 2037.86660 [27] & 685.34222 & 6.818 [01], 6.664 [27] & 4.14 & 0.75 & 0 & -- \\
56 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=268534931}{268534931} & 1398.29475 [03] & 2139.09941 [30] & 740.80465 & 5.829 [03], 6.133 [30] & 7.82 & 0.58 & 0 & 25.23 \\
57 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=269333648}{269333648} & 1538.52419 [08] & 2249.05416 [34] & 710.52997 & 4.162 [08], 4.032 [34] & 9.46 & 1.07 & 0 & 3.20 \\
58 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=275878706}{275878706} & 1621.08010 [11] & 2341.78257 [38] & 720.70247 & 6.544 [11], 5.320 [38] & 4.38 & 4.15 & 1 & 21.81 \\
59 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=279727635}{279727635} & 1343.22676 [01] & 2124.62930 [30] & 781.40254 & 7.181 [01], 6.789 [30] & 5.71 & 2.34 & 0 & -- \\
60 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=287204963}{287204963} & 1402.93640 [03] & 2132.33438 [30] & 729.39798 & 11.498 [03], 10.182 [30] & 4.73 & 1.05 & 0 & -- \\
61 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=289840544}{289840544} & 1331.28977 [01] & 2083.28790 [28] & 751.99813 & 2.702 [01], 1.997 [28] & 2.99 & 2.95 & 0 & 6.43 \\
62 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=290165539}{290165539} & 1332.75615 [01] & 2067.97094 [28] & 735.21479 & 13.627 [01], 15.056 [28] & 11.50 & 2.23 & 0 & 45.38 \\
63 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=292719109}{292719109} & 1499.70159 [07] & 2222.31933 [33] & 722.61775 & 2.859 [07], 2.677 [33] & 9.08 & 1.02 & 0 & 2.50 \\
64 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=294097549}{294097549} & 1657.74149 [13] & 2256.34250 [35] & 598.60101 & 1.977 [13], 1.426 [35] & 7.96 & 0.45 & 0 & 4.14 \\
65 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=296737508}{296737508} & 1538.00622 [08] & 2271.99796 [35] & 733.99174 & 2.021 [08], 1.854 [35] & 5.65 & 0.50 & 0 & 1.12 \\
66 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=300394149}{300394149} & 1576.88642 [10] & 2325.42588 [37] & 748.53947 & 2.051 [10], 2.195 [37] & 13.40 & 0.61 & 0 & 4.92 \\
67 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=303317324}{303317324} & 1365.17582 [02] & 2104.34337 [29] & 739.16755 & 1.360 [02], 1.323 [29] & 5.74 & 0.28 & 0 & 1.16 \\
68 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=304339227}{304339227} & 1673.33918 [13] & 2388.01911 [39] & 714.67993 & 0.522 [13], 0.464 [39] & 5.79 & 0.28 & 0 & 2.19 \\
69 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=306249066}{306249066} & 1593.97611 [10] & 2326.51397 [37] & 732.53786 & 7.873 [10], 7.061 [37] & 4.03 & 1.00 & 0 & 7.34 \\
70 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=313671132}{313671132} & 1604.35452 [11] & 2337.72693 [38] & 733.37241 & 3.408 [11], 3.506 [38] & 5.70 & 0.74 & 0 & 7.02 \\
71 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=317923092}{317923092} & 1479.81772 [06] & 2209.42617 [33] & 729.60845 & 4.358 [06], 6.715 [33] & 12.96 & 6.31 & 0 & 35.10 \\
72 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=323295479}{323295479} & 1622.92483 [11] & 2365.44036 [39] & 742.51554 & 8.727 [11], 8.609 [39] & 6.51 & 1.01 & 0 & 2.43 \\
73 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=332697924}{332697924} & 1445.74977 [05] & 2178.22194 [32] & 732.47218 & 1.042 [05], 1.423 [32] & 6.63 & 0.44 & 0 & 5.60 \\
74 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=333736132}{333736132} & 1551.55292 [09] & 2283.54681 [36] & 731.99390 & 15.856 [09], 16.440 [36] & 2.96 & 0.95 & 0 & 13.92 \\
75 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=339399841}{339399841} & 1662.10984 [13] & 2043.59486 [27] & 381.48503 & 4.773 [13], 6.471 [27] & 6.66 & 1.13 & 0 & -- \\
76 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=349091983}{349091983} & 1603.10253 [11] & 2152.16754 [31] & 549.06501 & 8.301 [11], 8.133 [31] & 9.52 & 4.91 & 0 & -- \\
77 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=366322247}{366322247} & 1618.29549 [11] & 2352.41070 [38] & 734.11521 & 4.569 [11], 4.223 [38] & 2.87 & 12.83 & 0 & -- \\
78 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=381553868}{381553868} & 1677.32594 [13] & 2367.57869 [39] & 690.25274 & 5.653 [13], 6.030 [39] & 6.49 & 1.12 & 0 & 9.94 \\
79 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=393229954}{393229954} & 1446.79953 [05] & 2204.55168 [33] & 757.75214 & 8.172 [05], 6.652 [33] & 2.67 & 0.79 & 0 & 12.97 \\
80 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=394340183}{394340183} & 1664.84261 [13] & 2389.11243 [39] & 724.26982 & 11.255 [13], 10.820 [39] & 8.65 & 1.04 & 0 & 6.77 \\
81 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=396720998}{396720998} & 1399.21966 [03] & 2176.27178 [32] & 777.05212 & 6.360 [03], 6.082 [32] & 4.33 & 0.13 & 0 & -- \\
82 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=404518509}{404518509} & 1431.26615 [04] & 2134.88294 [30] & 703.61679 & 0.842 [04], 0.598 [30] & 5.02 & 0.24 & 0 & 0.93 \\
83 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=412386707}{412386707} & 1493.95365 [07] & 2240.57066 [34] & 746.61701 & 3.442 [07], 3.587 [34] & 5.23 & 1.08 & 0 & 6.18 \\
84 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=437293313}{437293313} & 1578.44737 [10] & 2328.08914 [37] & 749.64177 & 9.891 [10], 8.462 [37] & 6.58 & 0.81 & 0 & -- \\
85 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=439491923}{439491923} & 1405.41115 [03] & 2116.79038 [30] & 711.37923 & 11.608 [03], 11.766 [30] & 6.70 & 1.33 & 0 & -- \\
86 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=442893494}{442893494} & 1472.65885 [06] & 2194.38454 [32] & 721.72570 & 5.776 [06], 6.458 [32] & 7.70 & 1.01 & 0 & -- \\
87 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=457649900}{457649900} & 1606.96984 [11] & 2355.79522 [38] & 748.82538 & 2.857 [11], 2.945 [38] & 7.61 & 4.54 & 0 & 13.11 \\
88 & \href{https://exofop.ipac.caltech.edu/tess/target.php?id=466206508}{466206508} & 1679.34576 [13] & 2054.97133 [27] & 375.62557 & 11.214 [13], 9.274 [27] & 8.03 & 1.24 & 0 & 12.81 \\
\bottomrule
%\label{tab:candidate_events}
\end{longtable}
\end{landscape}








\clearpage
\twocolumn




==> working-space.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
